Model Reduction for Multi-Scale Transport Problems using Model-form Preserving Least-Squares Projections with Variable Transformation

A projection-based formulation is presented for non-linear model reduction of problems with extreme scale disparity. The approach allows for the selection of an arbitrary, but complete, set of solution variables while preserving the structure of the governing equations. Least-squares-based minimization is leveraged to guarantee symmetrization and discrete consistency with the full-order model (FOM). Two levels of scaling are used to achieve the conditioning required to effectively handle problems with extremely disparate physical phenomena, characterized by extreme stiffness in the system of equations. The formulation -- referred to as model-form preserving least-squares with variable transformation (MP-LSVT) -- provides global stabilization for both implicit and explicit time integration schemes. To achieve computational efficiency, a pivoted QR decomposition is used with oversampling, and adapted to the MP-LSVT method. The framework is demonstrated in representative two- and three-dimensional reacting flow problems, and the MP-LSVT is shown to exhibit improved stability and accuracy over standard projection-based ROM techniques. Physical realizability and local stability are promoted by enforcing limiters in both temperature and species mass fractions. These limiters are demonstrated to be important in eliminating regions of spurious burning, thus enabling the ROMs to provide accurate representations of the heat release rate and flame propagation speed. In the 3D application, it is shown that more than two orders of magnitude acceleration in computational efficiency can be achieved, while also providing reasonable future-state predictions. A key contribution of this work is the development and demonstration of a comprehensive ROM formulation that targets highly challenging multi-scale transport-dominated problems.

==> Reviewer1.tex <==

\setcounter{page}{1}

\noindent \textbf{Reviewer 1}

In the response to reviewers, the authors answered five of my questions. While, in my review report, there are seven questions. Therefore, I would like to ask the authors to provide another minor revision to address the two concerns that are absent in this version. Furthermore, I suggest that in the response to reviewers, the authors clearly mention the page, paragraph, and line number of the corresponding revision. 

{\color{blue} We apologize for the oversight on not including the responses to the last two comments that the reviewer made. We have included our responses to the reviewer's two comments below.}

\begin{enumerate}

\item As pointed out in the Introduction, the projection-based ROMs suffer from accuracy and
stability issues, which may arise from the inherent lack of numerical stability of the projection, model truncation and simplifications of model equations. Recent studies have shown
that improving the numerical stability of the ROM (such as ensuring structure-preserving),
or adding memory closure term based on the Mori-Zwanzig formalism, improves the stability and accuracy of the projection-based ROM. The work has been done in this manuscript is improving the ROM from the numerical
point of view. Could the authors comment on the potential use of memory closure for the
SP-LSVT?

{\color{blue} The authors agree that the use of memory closure can be beneficial for the ROM method presented in the current paper, especially in mitigating the spurious oscillations reported in the paper. Indeed, the third author has  explored this topic~\footnote{ Parish, Eric J., and Karthik Duraisamy. "Non-Markovian closure models for large eddy simulations using the Mori-Zwanzig formalism." Physical Review Fluids 2.1 (2017): 014604.} As discussed in the paper, the major cause of these spurious oscillations is due to the lack of resolution using limited number of POD modes, which can be greatly improved adding memory closure term to the ROM. Indeed, we have  attempted a Markovian approximation to the Mori-Zwanzing memory kernel in the context of ROMs.~\footnote{Parish, Eric J., Christopher R. Wentland, and Karthik Duraisamy. "The Adjoint Petrov–Galerkin method for non-linear model reduction." Computer Methods in Applied Mechanics and Engineering 365 (2020): 112991}.}

\item I suggest the authors to give a definition of the heat release when presenting the numerical results, as readers may not be familiar with the meaning of heat release in rocket
combustion.

{\color{blue}This is a great suggestion. Per reviewer's request, a definition of the heat release rate has been added in Page 19 (first paragraph) in blue.}


\end{enumerate}

==> Reviewer2.tex <==
\noindent \textbf{Reviewer 2}

\noindent The authors made significant revisions to the paper, largely addressing my concerns. I have two minor comments:

\begin{enumerate}
\item In the Highlights, point 1., the term ``structure-preserving" should be made more specific, or replaced with something else, as ``structure-preserving" in the ROM community is a loaded term that refers to Hamiltonian mechanics. Maybe ``preserving the model form" or so? This should also be re-evaluated to be clarified in several places in the manuscript.

{\color{green} The authors agree with the reviewer's comment regarding the possible confusion from the terminology "structure-preserving". Therefore, we have replaced "structure-preserving" with "model-form preserving" for clarifications in the highlights and also in the manuscript. The changes are highlighted in green in the revision throughout the entire manuscript and also include legends in Figs.4, 5, 6(c), 9, 10, and 14.}

\item In Highlights, item 3, ``discrete-time" should be added.

{\color{green} Per reviewer's comment, it has been added to the Highlights, marked in green in item 3.}
\end{enumerate}


==> figures/FullOrderModel.tex <==


\section{Full-Order Model  and Time Discretization}
\label{fom}


We represent the governing equations of the full-order model as a generic dynamical system
\begin{equation}
    \frac{\text{d}\mathbf{q}}{\dTimeVar}=\mathbf{f}\left(\mathbf{q}, \timeVar \right), \ \ \mathbf{q}(0) = \mathbf{q}_0,
    \label{cfd:discretized}
\end{equation}
where $\timeVar \in [0,T]$ is the solution time, $\mathbf{q}: [0, T] \rightarrow {\mathbb{R}^{\numDOF}}$ is the vector of state variables, and $\mathbf{f}: \mathbb{R}^{\numDOF} \times [0,T] \rightarrow \mathbb{R}^{\numDOF}$ is a (potentially non-linear) function. While our formulation is general,  demonstrations are performed on dynamical systems that are derived from a spatial discretization of partial differential equations. For instance, in a finite volume setting,  $\numDOF = \numCells \times\numVars$, where $\numCells$ is the total number of finite volumes  and $\numVars$ is the number of state variables in each volume. The function $\mathbf{f}$ would thus represent surface fluxes, source terms, and body forces arising from the spatial discretization of the governing equations. Equation~\ref{cfd:discretized} (or its fully-discrete counterpart) is referred to as the full-order model (FOM), and for reasonably complex systems with well-refined spatial discretizations, the dimension $\numDOF$ may be $O(10^5 \; \text{-} \; 10^8)$.
%\subsection{Fully-discrete Representation of Governing Equations}

Two classes of time-discretization methods to solve Eq.~\ref{cfd:discretized} are introduced: linear multi-step methods and Runge--Kutta methods.

\subsection{Linear Multi-step Methods}
\label{LinearMultistep}
The solution to the governing equations (Eq.~\ref{cfd:discretized}) can be computed using linear multi-step methods, the $\itermaxLinMS$-step version of which can be expressed as
\begin{equation}
    \mathbf{q}^{\iterIdx}+\sum^{\itermaxLinMS}_{j=1}\alpha_j \mathbf{q}^{\iterIdx-j} = \dt \beta_0\mathbf{f}\left(\mathbf{q}^\iterIdx,\timeVar^\iterIdx\right) + \dt \sum^{\itermaxLinMS}_{j=1}\beta_j\mathbf{f}\left(\mathbf{q}^{\iterIdx-j},\timeVar^{\iterIdx-j}\right),
    %\mathbf{q}(\mathbf{q}_p^{n})+\sum^{k}_{j=1}\alpha_j \mathbf{q}(\mathbf{q}_p^{n-j})=\Delta \text{t}\beta_0\mathbf{f}\left(\mathbf{q}_p^n,\text{t}^n\right)+\Delta \text{t}\sum^{k}_{j=1}\beta_j\mathbf{f}\left(\mathbf{q}_p^{n-j},\text{t}^{n-j}\right),
    \label{cfd:LinearMultiStep}
\end{equation}
where $\dt \in \mathbb{R}^{+}$ is the physical time step for the numerical solution, and the coefficients $\alpha_j$, $\beta_j \in \mathbb{R}$ are determined  based on $\itermaxLinMS$. If $\beta_0 = 0$ , the method is explicit; otherwise, the method is implicit. The FOM equation residual $\mathbf{r}: \mathbb{R}^{\numDOF} \rightarrow \mathbb{R}^{\numDOF}$ is  defined as
\begin{equation}
    \mathbf{r}(\mathbf{q}^\iterIdx) \triangleq \mathbf{q}^{\iterIdx}+\sum^{\itermaxLinMS}_{j=1}\alpha_j \mathbf{q}^{\iterIdx-j} - \dt \beta_0\mathbf{f}\left(\mathbf{q}^\iterIdx,\timeVar^\iterIdx\right) - \dt \sum^{\itermaxLinMS}_{j=1} \beta_j \mathbf{f} \left( \mathbf{q}^{\iterIdx-j}, \timeVar^{\iterIdx-j} \right).
    %\mathbf{r}(\mathbf{q}_p^n) = \mathbf{q}(\mathbf{q}_p^{n})+\sum^{k}_{j=1}\alpha_j \mathbf{q}(\mathbf{q}_p^{n-j})-\Delta \text{t}\beta_0\mathbf{f}\left(\mathbf{q}_p^n,\text{t}^n\right)-\Delta \text{t}\sum^{k}_{j=1}\beta_j\mathbf{f}\left(\mathbf{q}_p^{n-j},\text{t}^{n-j}\right).
    \label{EqRes:LinearMultiStep}
\end{equation}
The state variables, $\mathbf{q}^\iterIdx$, are solved for at each time step so that $\mathbf{r}(\mathbf{q}^\iterIdx) = 0$.

% Similarly, we can derive the equation residual for Eq.~\ref{cfd:discretized_qp_ge} solved by linear multistep method,
% \begin{equation}
%     \mathbf{\hat{r}}(\mathbf{q}_p^n) = \mathbf{q}_p^{n}+\sum^{k}_{j=1}\alpha_j \mathbf{q}_p^{n-j}-\Delta \text{t}\beta_0\mathbf{\hat{f}}\left(\mathbf{q}_p^n,\text{t}^n\right)-\Delta \text{t}\sum^{k}_{j=1}\beta_j\mathbf{\hat{f}}\left(\mathbf{q}_p^{n-j},\text{t}^{n-j}\right).
%     \label{EqRes_qp:LinearMultiStep}
% \end{equation}

\subsection{Runge--Kutta Methods}
\label{RK}
Alternatively, the governing equations can be solved numerically using the $\itermaxRK$-stage Runge--Kutta method
\begin{equation}
    \mathbf{q}^{\iterIdx}=\mathbf{q}^{\iterIdx-1} + \dt \sum^{\itermaxRK}_{j=1} b_j \mathbf{s}_j,
    %\mathbf{q}(\mathbf{q}_p^{n})=\mathbf{q}(\mathbf{q}_p^{n-1})+\Delta \text{t}\sum^{s}_{j=1}b_j{\mathbf{s}_j},
    \label{cfd:RK}
\end{equation}
where $\mathbf{s}_1 = \mathbf{f}\left(\mathbf{q}^{\iterIdx-1},\timeVar^{\iterIdx-1}\right)$ and
\begin{equation}
    \mathbf{s}_j = \mathbf{f}\left(\mathbf{q}^{\iterIdx-1} + \dt \sum^{j-1}_{m=1} a_{jm}{\mathbf{s}_m}, \timeVar^{\iterIdx-1} + c_j \dt \right),
    %\mathbf{s}_j = \mathbf{f}\left(\mathbf{q}_p^{n-1}+\Delta \text{t}\sum^{j-1}_{m=1}a_{jm}{\mathbf{s}_m},\text{t}^{n-1}+c_j\Delta\text{t}\right),
    \label{cfd:RK_stage}
\end{equation}
and the coefficients, $a_{jm}$, $b_j$, $c_j \in \mathbb{R}$ are determined for different Runge--Kutta methods. The methods are explicit if $a_{jm} = 0$, $\forall \; m \geq j$, and are diagonally implicit if $a_{jm} = 0$, $\forall \; m > j$.  The FOM equation residual is defined as
\begin{equation}
    \mathbf{r}(\mathbf{q}^\iterIdx) \triangleq \mathbf{q}^{\iterIdx} - \mathbf{q}^{\iterIdx-1} - \dt \sum^{\itermaxRK}_{j=1} b_j \mathbf{s}_j.
    %\mathbf{r}(\mathbf{q}_p^n) = \mathbf{q}(\mathbf{q}_p^{n}) - \mathbf{q}(\mathbf{q}_p^{n-1}) - \Delta\text{t}\sum^{s}_{j=1}b_j{\mathbf{s}_j}.
    \label{EqRes:RK}
\end{equation}
where, again, the solution variables, $\mathbf{q}_p^\iterIdx$, are solved at each time step such that $\mathbf{r}(\mathbf{q}^\iterIdx) = 0$.

% Similarly, we can derive the equation residual for Eq.~\ref{cfd:discretized_qp_ge} solved by $s$-stage Runge–Kutta method,
% \begin{equation}
%     \mathbf{\hat{r}}(\mathbf{q}_p^n) = \mathbf{q}_p^{n} - \mathbf{q}_p^{n-1} - \Delta\text{t}\sum^{s}_{j=1}b_j{\mathbf{\hat{s}}_j}.
%     \label{EqRes_qp:RK}
% \end{equation}
% where $\mathbf{\hat{s}}_1 = \mathbf{\hat{f}}\left(\mathbf{q}_p^{n-1},\text{t}^{n-1}\right)$ and,
% \begin{equation}
%     \mathbf{\hat{s}}_j = \mathbf{\hat{f}}\left(\mathbf{q}_p^{n-1}+\Delta \text{t}\sum^{j-1}_{m=1}a_{jm}{\mathbf{\hat{s}}_m},\text{t}^{n-1}+c_j\Delta\text{t}\right),
%     \label{cfd_qp:RK_stage}
% \end{equation}

==> figures/HyperReduction.tex <==
\subsection{Hyper-reduction}
\label{hyper_reduction}

\begin{comment}
Even though projection-based ROMs lead to discrete systems of much lower dimension ($n_p \ll N$), the evaluations of the non-linear terms $\mathbf{f}(\cdot)$ in the equations remains a bottleneck as it involves $O(N)$ operations. % (e.g. $\mathbf{f}$ in Eq.~\ref{rom:galerkin_ode}). This is generally referred to as the ``lifting bottleneck,'' wherein the low-dimensional state $\hat{\mathbf{q}}_r$ must be ``lifted'' to the full-dimensional state $\tilde{\mathbf{q}}_p$ before evaluating the non-linear terms. Unfortunately, computing the non-linear terms is often the most computationally expensive step of solving ODEs of complex systems (e.g. combusting flow). This issue, along with expensive projection operations which scale with $N$, usually results in projection-based ROMs on non-linear systems being \textit{more} computationally expensive than the original FOM calculation.
A popular method of circumventing this problem is the discrete empirical interpolation method (DEIM)~\cite{1}, a technique which uses sparse samples to reconstruct the full-dimensional reconstruction of $\mathbf{f}(\cdot)$. 
%\begin{comment}
\subsubsection{Hyperreduced SP-LSVT ROMs: Physical Time}
We begin by reformulating the fully-discrete ROM residual for linear multistep time integrators in physical time (Eq.~\ref{EqRes:LinearMultiStep_qp}), given by,
\begin{align}
\begin{split}
    \overline{\mathbf{r}}(\tilde{\mathbf{q}}^k_p) &= \mathbf{q} (\tilde{\mathbf{q}}^{k} ) + \sum^{k}_{j=1} \alpha_j \mathbf{q} (\tilde{\mathbf{q}}^{n-j} ) - \mathbf{U} \left(\mathbf{S}^T \mathbf{U}\right)^{-1} \mathbf{S}^T \left[ \Delta \text{t} \beta_0 \mathbf{f} \left( \tilde{\mathbf{q}}^k, \text{t}^n \right) + \Delta \text{t} \sum^{k}_{j=1} \beta_j \mathbf{f} \left( \tilde{\mathbf{q}}^{n-j}, \text{t}^{n-j} \right) \right], \\
    &= \mathbf{q} (\tilde{\mathbf{q}}^{k}) + \sum^{k}_{j=1} \alpha_j \mathbf{q} (\tilde{\mathbf{q}}^{n-j} ) - \Delta \text{t} \beta_0 \overline{\mathbf{f}} \left( \tilde{\mathbf{q}}^k, \text{t}^n \right) - \Delta \text{t} \sum^{k}_{j=1} \beta_j \overline{\mathbf{f}} \left( \tilde{\mathbf{q}}^{n-j}, \text{t}^{n-j} \right).
\end{split}
\end{align}
The accompanying test basis, originally given by Eq.~\ref{rom:lspg_w_LinearMultistep}, is simply reformulated as,
\begin{equation}
    \hat{\overline{\mathbf{W}}}^k = \mathbf{P} \left(\hat{\boldsymbol{\Gamma}}^k - \Delta \text{t} \beta_0 \hat{\overline{\mathbf{J}}}^k \hat{\boldsymbol{\Gamma}}^k \right)\mathbf{H}^{-1}\mathbf{\hat{V}},
\end{equation}
resulting in the familiar, symmetrized linear system which governs the evolution of the hyperreduced ROM,
\begin{equation}
    (\mathbf{\hat{\overline{W}}}^{k-1})^T \mathbf{\hat{\overline{W}}}^{k-1} (\mathbf{\hat{q}}^k_r-\mathbf{\hat{q}}^{k-1}_r) + (\mathbf{\hat{\overline{W}}}^{k-1})^T \mathbf{P} \overline{\mathbf{r}}(\mathbf{\tilde{q}}^{k-1}_p) = 0.
\end{equation}

\subsubsection{Hyperreduced SP-LSVT ROMs: Dual Time-stepping}
Again substituting the interpolated non-linear function $\mathbf{f}$ and its Jacobians, the ROM residual for dual time-stepping with linear multistep time integration (Eq.~\ref{RomRes:LinearMultiStep_qp_DualTime}) is reformulated as,
\begin{align}
\begin{split}
    \overline{\mathbf{r}}_p(\tilde{\mathbf{q}}^k_p) &= \left[\left(\frac{1}{\Delta\tau} + 1\right) \boldsymbol{\Gamma}^{k-1} - \beta_0 \mathbf{U} \left(\mathbf{S}^T \mathbf{U}\right)^{-1} \mathbf{S}^T \hat{\mathbf{J}}^{k-1} \hat{\boldsymbol{\Gamma}}^{k-1} \right] \Delta \text{t} (\mathbf{q}_p^{k} - \mathbf{q}_p^{k-1}) + \overline{\mathbf{r}}(\mathbf{q}_p^{k-1}), \\
    &= \left[ \left( \frac{1}{\Delta\tau} + 1 \right) \boldsymbol{\Gamma}^{k-1} - \beta_0 \hat{\overline{\mathbf{J}}}^{k-1} \hat{\boldsymbol{\Gamma}}^{k-1}  \right] \Delta\text{t} (\mathbf{q}_p^{k} - \mathbf{q}_p^{k-1}) + \overline{\mathbf{r}} (\mathbf{q}_p^{k-1}),
\end{split}
\end{align}
Similarly, the test basis (Eq.~\ref{rom:lspg_w_qp_DualTime}) is written
\begin{equation}
    \mathbf{\tilde{\overline{W}}}^k = \mathbf{P} \left[\left(\frac{1}{\Delta\tau} + 1\right) \hat{\boldsymbol{\Gamma}}^{k-1} - \beta_0 \hat{\mathbf{J}}^{k-1} \hat{\boldsymbol{\Gamma}}^{k-1} \right] \Delta \text{t} \mathbf{H}^{-1} \mathbf{\hat{V}}.
\end{equation}
%\end{comment}

As mentioned previously, it is not strictly required that $n_s = n_d$. In fact, it has been shown by Peherstorfer et al.~\cite{4} that increasing $n_d$ and maintaining $n_s = n_d$ can lead to greatly degr
\end{comment}

Even though projection-based ROMs lead to discrete systems of much lower dimension ($\numSolModes \ll \numDOF$), the evaluations of the non-linear terms in the equations remain a bottleneck as they involve $O(\numDOF)$ operations. % (e.g. $\mathbf{f}$ in Eq.~\ref{rom:galerkin_ode}). This is generally referred to as the ``lifting bottleneck,'' wherein the low-dimensional state $\hat{\mathbf{q}}_r$ must be ``lifted'' to the full-dimensional state $\tilde{\mathbf{q}}_p$ before evaluating the non-linear terms. Unfortunately, computing the non-linear terms is often the most computationally expensive step of solving ODEs of complex systems (e.g. combusting flow). This issue, along with expensive projection operations which scale with $N$, usually results in projection-based ROMs on non-linear systems being \textit{more} computationally expensive than the original FOM calculation.
A popular method to circumvent this problem is the discrete empirical interpolation method (DEIM)~\cite{chaturantabut2010nonlinear}, or its oversampled analogue, gappy POD~\cite{gappyPOD}. These methods use sparse samples and data-driven interpolation to develop a full reconstruction of the non-linear function at non-sampled elements. This approximation of the non-linear function by gappy POD is given by the formulation

%Even though projection-based ROMs  lead to discrete systems of much lower dimension ($\numSolModes \ll \numDOF$), the evaluations of the non-linear terms in the equations (e.g. $\mathbf{f}$ in Eq.~\ref{rom:galerkin_ode} and $\mathbf{r}$ in Eq.~\ref{rom:lspg_proj}) still require operations on the order of $\numDOF$, the dimension of the original FOM. Therefore, hyper-reduction of these non-linear terms is necessary via sparse sampling methods, which compute a small subset of the non-linear terms. 
%The DEIM approach yields a reconstructed residual 
\begin{equation}
\mathbf{\overline{r}} \approx \mathbf{U} (\mathbf{S}^T \mathbf{U})^{+}  \mathbf{S}^T \mathbf{r},
\label{rom:deim_approx}
\end{equation}
where $\mathbf{S} \in \mathbb{R}^{\numDOF \times \numSamps}$ is a selection operator that samples $n_s$ columns (i.e. sampling points) of the identity matrix, $\mathbf{I} \in \mathbb{R}^{\numDOF \times \numDOF}$, and $\mathbf{U} \in \mathbb{R}^{\numDOF \times \numResModes}$ is a basis set used to approximate the non-linear term, $\mathbf{r}$. Typically, $\mathbf{U}$ is constructed via POD from snapshots of $\mathbf{r}$. However, the authors have found that setting $\mathbf{U}$ to the trial POD basis $\mathbf{V}$ in Eq.~\ref{pod:expansion_consv} or $\mathbf{\hat{V}}$ in Eq.~\ref{pod:expansion_qp} also produces excellent approximations; this method is used for all results presented in this paper. Further, although it is not strictly required that $\numResModes = \numSolModes$, this is true for all cases presented in this paper.

\begin{comment}
The same approximation can be extended to Jacobians of the non-linear term, exemplified by
\begin{equation}
    \mathbf{\tilde{\overline{J}}} \approx \frac{ \partial \mathbf{U} (\mathbf{S}^T \mathbf{U})^{+} \mathbf{S}^T \mathbf{r}(\mathbf{\tilde{q}}_p)}{\partial\mathbf{\hat{q}}_r} = \mathbf{U} (\mathbf{S}^T \mathbf{U})^{+} \mathbf{S}^T \frac{ \partial \mathbf{r}(\mathbf{\tilde{q}}_p)}{\partial\mathbf{\hat{q}}_r} = \mathbf{U} (\mathbf{S}^T \mathbf{U})^{+} \mathbf{S}^T \tilde{\mathbf{J}}
\end{equation}
Thus, only $\numSamps$ rows of the Jacobian $\tilde{\mathbf{J}}$ are sampled.
\end{comment}

By applying sparse sampling and interpolation, the cost of evaluating the non-linear term $\mathbf{r}$ now scales with $\numSamps$, where $\numSamps \ll \numDOF$. %This has effectively eliminated the lifting bottleneck, of course at the cost of any error introduced by the interpolation. 
It has to be recognized that for coupled dynamical systems -- such as those generated via the spatial discretization of a PDE -- $\mathbf{S}^T \mathbf{r}(\mathbf{q}_p) \neq \mathbf{r}(\mathbf{S}^T \mathbf{q}_p)$; additional elements of $\mathbf{r}$ must be evaluated to compute the sub-sampled non-linear term. The scalable implementation of sparse sampling, especially critical for complex multi-scale problems, is discussed in greater detail in~\ref{appendix:hyperreductionDetails}. In the current work, the first $\numResModes$ sampling points are chosen using the rank-revealing QR algorithm suggested in Ref.~\cite{drmac_qdeim}. The remaining $\numSamps - \numResModes$ oversampling points are selected via a uniform random distribution, following evaluations performed by Peherstorfer et al.~\cite{PeherstorferODEIM}, which demonstrated that randomized oversampling can stabilize DEIM and is necessary especially when noise (e.g. from turbulence or numerical inaccuracies) is present in the problem.


%By applying DEIM to approximate the nonlinear term, $\mathbf{\hat{f}}$, the Galerkin ROM ODE (Eq.~\ref{rom:galerkin_ode}) becomes,
%\begin{equation}
%    \frac{\text{d}{\mathbf{q}_r}}{\text{dt}} = \mathbf{V}^T \mathbf{H}^2 \mathbf{U} (\mathbf{S}^T \mathbf{U})^{+} \mathbf{S}^T \mathbf{f}\left( \mathbf{V}\mathbf{q}_r,t\right),
%    \label{rom:galerkin_ode_deim}
%\end{equation}
%where $\mathbf{V}^T \mathbf{H}^2 \mathbf{U} (\mathbf{S}^T \mathbf{U})^{+} \in \mathbb{R}^{n_p \times n_s}$ can be precomputed offline. Similarly, the LSPG ROM with DEIM approximation of $\mathbf{r}$ becomes,
%\begin{equation}
 %   (\mathbf{S}^T \mathbf{W}^n)^T [(\mathbf{S}^T \mathbf{U})^{+}]^T (\mathbf{S}^T \mathbf{U})^{+} \mathbf{S}^T \mathbf{P}^2 \mathbf{r}(\mathbf{V}\mathbf{q}^n_r) = 0,
 %   \label{rom:slspg_proj_deim}
%\end{equation}


We now extend the gappy POD formulation to the SP-LSVT ROMs in a fashion similar to that of Carlberg et. al~\cite{carlberg2013gnat}. We begin by applying sparse sampling and interpolation to the non-linear equation residual $\mathbf{r}$ in Eq.~\ref{rom:lspg_def} 
\begin{equation}
    \tilde{\mathbf{q}}^n_p \triangleq  \arg \min_{\tilde{\mathbf{q}}^n_p \in \textrm{Range}(\mathbf{\hat{V}})} \norm{\mathbf{U} (\mathbf{S}^T \mathbf{U})^{+}\mathbf{S}^T\mathbf{P}\mathbf{r}(\mathbf{\tilde{q}}^n_p)}^2.
    \label{rom:lspg_def_deim}
\end{equation}
The resulting test basis $\mathbf{\hat{W}}^\iterIdx$  is then given by
\begin{equation}
    \mathbf{\hat{\overline{W}}}^\iterIdx =  \frac{ \partial \mathbf{U} (\mathbf{S}^T \mathbf{U})^{+}\mathbf{S}^T\mathbf{P}\mathbf{r}(\mathbf{\tilde{q}}^\iterIdx_p)}{\partial\mathbf{\hat{q}}^\iterIdx_r} = \mathbf{U} (\mathbf{S}^T \mathbf{U})^{+}\mathbf{S}^T \frac{ \partial \mathbf{P}\mathbf{r}(\mathbf{\tilde{q}}^\iterIdx_p)}{\partial\mathbf{\hat{q}}^\iterIdx_r} = \mathbf{U} (\mathbf{S}^T \mathbf{U})^{+}\mathbf{S}^T \mathbf{\hat{W}}^\iterIdx.
    \label{rom:lspg_w_deim}
\end{equation}
Thus, only $\numSamps$ rows of the test basis $\mathbf{\hat{W}}^n$ must be evaluated. This is yet another major step in reducing the number of necessary computations. 

With the approximated test basis in hand, the SP-LSVT ROM in physical time (Eq.~\ref{rom:lspg_proj}) becomes
\begin{equation}
 (\mathbf{\hat{\overline{W}}}^\iterIdx)^T \mathbf{U} (\mathbf{S}^T \mathbf{U})^{+}\mathbf{S}^T\mathbf{P}\mathbf{r}(\mathbf{\tilde{q}}^\iterIdx_p) = 0,
 \label{rom:lspg_proj_hyper}
\end{equation}
and, noting that $\mathbf{U}^T \mathbf{U} = \mathbf{I}$ by orthonormality, we arrive at the final form of the ROM
\begin{equation}
    (\mathbf{S}^T \mathbf{\hat{W}}^\iterIdx)^T [(\mathbf{S}^T \mathbf{U})^{+}]^T (\mathbf{S}^T \mathbf{U})^{+} \mathbf{S}^T \mathbf{P} \mathbf{r}(\mathbf{\tilde{q}}^\iterIdx_p) = 0
    \label{rom:lspg_proj_deim}
\end{equation}
where $[(\mathbf{S}^T \mathbf{U})^{+}]^T (\mathbf{S}^T \mathbf{U})^{+} \in \mathbb{R}^{\numSamps \times \numSamps}$ can be precomputed offline. Similarly, applying sparse sampling and interpolation technique to $\mathbf{r}_p$ in Eq.~\ref{rom:lspg_def_dualtime}, the SP-LSVT ROM in pseudo-time (Eq.~\ref{rom:lspg_proj_dualtime}) is given by
\begin{equation}
    (\mathbf{S}^T \mathbf{\tilde{W}}^k)^T [(\mathbf{S}^T \mathbf{U})^{+}]^T (\mathbf{S}^T \mathbf{U})^{+} \mathbf{S}^T \mathbf{P} \mathbf{r}_p(\mathbf{\tilde{q}}^\subIdx_p) = 0.
    \label{rom:lspg_proj_deim_pseudo}
\end{equation}

%Derivations for these formulation applied to linear multi-step and Runge--Kutta time integrators are provided in~\ref{appendix:hyperreductionDetails}.

==> figures/LSPG-VT.tex <==
\section{Structure-preserving Model Reduction for Transformed Solution Variables}
\label{SPLSPG}
In this section, we introduce the structure-preserving least-squares with variable transformation (SP-LSVT) ROM formulation. Since the targeted applications are complex multi-scale problems, this formulation involves a number of steps which are detailed below. %This method is designed to preserve the conservative form of the governing equations under transformations of the solution variables.

\subsection{Semi-discrete Formulation  for Transformed Solution Variables}
\label{fom_qp}
It is typical to develop projection-based model reduction methods (Section~\ref{StandardROM}) for the state variables used  in the full order model. For instance, compressible flow ROMs are derived with the conservative variables (density, momentum, total energy, etc.) as the unknowns.   In many circumstances, motivated either by physical or numerical considerations, it can be beneficial to solve the governing equations based on an alternate set of variables, which we denote generally by $\mathbf{q}_p$. \st{For example, the Euler equations of compressible flow can be transformed to an alternate set of variables to simplify the non-linearity %~\cite{pettersson2014stochastic}. 
In reacting flows, $\mathbf{q}_p$ may be the primitive variables, which include pressure ($p$), velocities ($\mathbf{u}$), temperature ($T$) and species mass fraction ($Y_k$), as they allow for easier computation of thermal properties and provide more flexibility when extending applications to complex fluid problems like liquid and supercritical fluids. Further, directly updating quantities such as pressure and temperature at the time-step (or sub-iteration) level may be beneficial from the viewpoint of enforcing physical realizability (e.g. positivity) and robustness. 
We now describe a transformation to such a different, but complete, set of variables $\mathbf{q}_p$, while not sacrificing important properties such as conservation.} 

{\color{blue}
The following are representative examples of variable transformations that serve as inspirations for the present work:
\begin{enumerate}
   
\item Kramer and Willcox ~\cite{Kramer2019LiftAndLearn,KramerBalancedROM}, Swischuk et al.~\cite{Swischuk2020AIAAJ_LL} and Qian et al.~\cite{qian2020lift} define a coordinate transformation to rewrite the governing equations in quadratic form. This simplified structure is leveraged to develop non-intrusive - yet interpretable - ROM operators. 

\item Similarly, Pettersson et al.~\cite{pettersson2014stochastic} use the Roe variables~\cite{Roe1981} to simplify the non-linearity of the compressible Euler equations. The simplified equations are used to develop intrusive stochastic Galerkin techniques for uncertainty quantification.

\item In contrast to hand-crafted variable transformations above, Pan et al.~\cite{pan2020physics} and Champion et al.~\cite{champion2019data} use neural network-based autoencoders to discover a latent space in which the dynamics is linear.

\item In computational fluid dynamic solvers, actions such as solution reconstruction and slope-limiting~\cite{cfd1-1,cfd1-2} and time marching updates~\cite{cfd2,Pulliam} are performed in terms of non-conservative variables, rather than the  conserved variables. Directly updating quantities such as pressure and temperature at the time-step (or sub-iteration) level will be beneficial from the viewpoint of enforcing physical realizability (e.g. positivity) and robustness. In reacting flows,  a primitive variable formulation~\cite{HarvazinskiPoF} allows for easier computation of thermal properties and provides more flexibility when extending applications to complex fluid problems like liquid and supercritical fluids.

\end{enumerate}

{\color{blue}Influenced by the above examples, we describe a transformation to a different, but complete, set of state variables $\mathbf{q}_p$. In contrast to {\em lifting-based approaches (items 1,2,3 above)}, however, we do not sacrifice important properties such as conservation.}

We begin by re-writing Eq.~\ref{cfd:discretized} as
\begin{equation}
    \frac{\text{d}\mathbf{q}(\mathbf{q}_p)}{\dTimeVar}=\mathbf{f}\left(\mathbf{q}_p,\timeVar\right),
    \label{cfd:discretized_qp}
\end{equation}
where $\mathbf{q}$ $: \mathbb{R}^{\numDOF} \rightarrow \mathbb{R}^{\numDOF}$  and $\mathbf{f}$ $: \mathbb{R}^{\numDOF} \times [0,T] \rightarrow \mathbb{R}^{\numDOF}$ are functions of the solution variables, $\mathbf{q}_{p}$ $: [0, T] \rightarrow {\mathbb{R}^{\numDOF}}$. Note that, in general, computing $\mathbf{f}$ often requires a combination of the conserved and solution variables, and the notation here is simply one of convenience.  Defining the Jacobian of the transformation $\boldsymbol{\Gamma} \triangleq {\partial \mathbf{q}} / {\partial \mathbf{q}_p}$, applying the chain rule, and applying the left inverse of $\boldsymbol{\Gamma}$ results in the following equation
\begin{equation}
    \frac{\text{d}\mathbf{q}_p}{\dTimeVar}=\boldsymbol{\Gamma}^{-1}\mathbf{f}\left(\mathbf{q}_p, \timeVar \right) = \mathbf{f}_p\left(\mathbf{q}_p,\timeVar\right).
    \label{cfd:discretized_qp_ge}
\end{equation}
Although this is formally equivalent to Eq.\ref{cfd:discretized_qp} (assuming differentiability) in the semi-discrete setting, it will not be conservative in the fully-discrete setting. Thus, a more careful approach is required to formulate the discrete representation. %\crw{This will be addressed in Section~\ref{lspg-vt-pseudo}.}

With arbitrary solution variables, the fully-discrete FOM equation residual for linear multi-step method in Section~\ref{fom} becomes
\begin{equation}
    \mathbf{r}(\mathbf{q}_p^\iterIdx) = \mathbf{q}(\mathbf{q}_p^{\iterIdx})+\sum^{\itermaxLinMS}_{j=1}\alpha_j \mathbf{q}(\mathbf{q}_p^{\iterIdx-j}) - \dt \beta_0 \mathbf{f} \left( \mathbf{q}_p^\iterIdx, \timeVar^\iterIdx\right) - \dt \sum^{\itermaxLinMS}_{j=1} \beta_j\mathbf{f} \left(\mathbf{q}_p^{\iterIdx-j},\timeVar^{\iterIdx-j}\right).
    \label{EqRes:LinearMultiStep_qp}
\end{equation}
The fully discrete FOM equation residual for Runge--Kutta method with arbitrary solution variables becomes
\begin{equation}
    \mathbf{r}(\mathbf{q}_p^\iterIdx) = \mathbf{q}(\mathbf{q}_p^{\iterIdx}) - \mathbf{q}(\mathbf{q}_p^{\iterIdx-1}) - \dt \sum^{\itermaxRK}_{j=1} b_j \mathbf{s}_j,
    \label{EqRes:RK_qp}
\end{equation}
where $\mathbf{s}_1 \triangleq \mathbf{f}\left( \mathbf{q}_p^{\iterIdx-1}, \timeVar^{\iterIdx-1} \right)$ and
\begin{equation}
    \mathbf{s}_j = \mathbf{f}\left( \mathbf{q}_p^{\iterIdx-1} + \dt \sum^{j-1}_{m=1} a_{jm} \boldsymbol{\Gamma}_m^{-1}{\mathbf{s}_m}, \timeVar^{\iterIdx-1} + c_j \dt \right),
    \label{cfd:RK_stage_qp}
\end{equation}
with $\boldsymbol{\Gamma_1} \triangleq \boldsymbol{\Gamma}\left( \mathbf{q}_p^{\iterIdx-1},\timeVar^{\iterIdx-1}\right)$ and
\begin{equation}
    \boldsymbol{\Gamma_j} = \boldsymbol{\Gamma}\left( \mathbf{q}_p^{\iterIdx-1} + \dt \sum^{j-1}_{m=1}a_{jm} \boldsymbol{\Gamma}_m^{-1} \mathbf{s}_m, \timeVar^{\iterIdx-1} + c_j \dt \right).
    \label{cfd:GammaInv_qp}
\end{equation}

%In the remainder of this section, we derive the structure-preserving least-squares with variable transformation (SP-LSVT) ROM formulation, which preserves the structure of the conservative governing equations while allowing for the selection of arbitrary solution variables.

\subsection{Construction of POD Bases for Arbitrary Solution Variables}
%We first define POD bases derived for arbitrary non-conservative variables $\mathbf{q}_p$ (in contrast to the typical method of computing POD bases for the conservative variables $\mathbf{q}$, as in Section~\ref{pod:consv}). Given a database of FOM snapshots of the non-conservative variables, a POD basis may be calculated from  $\mathbf{q}'_p=\mathbf{q}_p-\mathbf{q}_{p,\text{ref}}$, where $\mathbf{q}_{p,\text{ref}}$ is a reference state extracted before POD basis calculation. An approximate solution, $\mathbf{\tilde{q}}_p \approx \mathbf{q}_p$, can be calculated,

Similar to Section~\ref{pod:consv}, the state $\mathbf{q}_p$ can be expressed in a trial space $\hat{\mathcal{V}} \triangleq \text{Range}(\mathbf{\hat{V}})$, where $\mathbf{\hat{V}} \in \mathbb{R}^{\numDOF \times \numSolModes}$ is the trial basis matrix. Define $\mathbf{q}_p^\prime(\timeVar) \triangleq \mathbf{q}_p(\timeVar) - \mathbf{q}_{p,\text{ref}}$, where $\mathbf{q}_{p,\text{ref}}$ is a reference state. Possible reference states include the initial FOM solution, $\mathbf{q}_{p,\text{ref}} = \mathbf{q}_p(\timeVar=\timeVar_0)$, or the time-averaged FOM solution, $\mathbf{q}_{p,\text{ref}} = \frac{1}{\Delta \text{T}}\int_{\timeVar_0}^{\timeVar_0+\Delta \text{T}} \mathbf{q}_p(\timeVar)\text{dt}$. 

We then seek a representation  $\mathbf{\tilde{q}}_p: [0,T] \rightarrow \hat{\mathcal{V}}$ such that
\begin{equation}
    \mathbf{H} (\mathbf{\tilde{q}}_p - \mathbf{q}_{p,\text{ref}} ) = \mathbf{\hat{V}}\mathbf{\hat{q}}_r.
    \label{pod:expansion_qp}
\end{equation}
Here, $\mathbf{\hat{q}}_r: [0,T] \rightarrow \mathbb{R}^{\numSolModes}$ is the reduced state, and $\numSolModes$ represents the number of trial basis modes. $\mathbf{\hat{V}}$ is the POD basis derived by the SVD from the FOM snapshots of $\mathbf{q}^\prime_p$, similar to the solution of Eq.~\ref{pod:orthogonality_consv}.
\begin{comment}, which is a solution to
\begin{equation}
  \min_{\mathbf{\hat{V}} \in \mathbb{R}^{\numDOF \times \numSolModes}} ||\mathbf{Q}_p-\mathbf{\hat{V}}\mathbf{\hat{V}}^T \mathbf{Q}_p||_F \ \ s.t. \ \ \mathbf{\hat{V}}^T \mathbf{\hat{V}} = \mathbf{I},
    \label{pod:orthogonality_qp}
\end{equation}
where $\mathbf{Q}_p$ is a data matrix in which each column is a snapshot of the solution  $ \mathbf{q}_p^\prime $.
\end{comment}

%And $\mathbf{\hat{V}}$ is the orthonormal POD basis,
%\begin{equation}
%   \mathbf{\hat{V}}^T \mathbf{\hat{V}} = \mathbf{I}.
%    \label{pod:orthogonality_qp}
%\end{equation}

Similar to Eq.~\ref{pod:normalization_consv}, a scaling matrix, $\mathbf{H} \in{\mathbb{R}^{\numDOF \times \numDOF}}$, must be applied to scale $\mathbf{q}'_p$ so that the numerical values of physical quantities (e.g. pressure, velocities, temperature and species mass fraction) have similar orders of magnitude in generating the POD basis. Again, in this work we choose to normalize all quantities by their $L^2$-norm
\begin{equation}
    \mathbf{H} = diag\left(\hat{\mathbf{H}}_1\ldots\hat{\mathbf{H}}_i\ldots\hat{\mathbf{H}}_{\numCells}\right),
    \label{pod:normalization_qp}
\end{equation} 
where $\hat{\mathbf{H}}_i=diag\left( \phi^{-1}_{1,norm}, \ldots , \phi^{-1}_{\numVars,norm} \right)$. Here, $\phi_{\normVarIdx,norm}$ represents the $\normVarIdx^{th}$ solution variable and
\begin{equation}
    \phi_{\normVarIdx,norm}={\frac{1}{\Delta \text{T}}\int^{t_0+\Delta \text{T}}_{\timeVar_0}\frac{1}{\Omega}\int_{\Omega}\phi'^2_\normVarIdx (\mathbf{x},\timeVar)\text{d}\mathbf{x}\text{dt}}.
\end{equation}

\subsection{Least-squares with Variable Transformation}
\label{lspg-vt}
As mentioned in Section~\ref{slspg_rom}, standard LSPG projection~\cite{Carlberg2017} requires an implicit, discrete-time representation of the governing equations. Otherwise, LSPG projection is equivalent to Galerkin projection. In this work, we seek to develop a structure-preserving least-squares formulation for an arbitrary selection of solution variables as in Eq.~\ref{cfd:discretized_qp}, and for both explicit and implicit time discretization schemes.

Our objective is to minimize the fully-discrete FOM equation residual $\mathbf{r}$, defined in Eqs.~\ref{EqRes:LinearMultiStep_qp} and~\ref{EqRes:RK_qp} with respect to the approximate solution variables, $\mathbf{\tilde{q}}_p = \mathbf{q}_{p,\text{ref}} + \mathbf{H}^{-1}\mathbf{\hat{V}}\mathbf{\hat{q}}_r$. It should be noted that for a fully-converged FOM $\mathbf{r}(\mathbf{q}^n_p) = 0$, but $\mathbf{r}(\mathbf{\tilde{q}}^n_p)$ is not necessarily equal to zero, as the ROM may be under-resolved. As in the LSPG technique, we seek to minimize the residual
\begin{equation}
    \tilde{\mathbf{q}}^n_p \triangleq  \arg \min_{\tilde{\mathbf{q}}^n_p \in \textrm{Range}(\mathbf{\hat{V}})} \norm{\mathbf{P}\mathbf{r}(\mathbf{\tilde{q}}^n_p)}^2,
    \label{rom:lspg_def}
\end{equation}
with the equation residual, $\mathbf{r}$, scaled by $\mathbf{P}$ such that each equation in $\mathbf{r}$ has similar contributions to the minimization problem in Eq.~\ref{rom:lspg_def}. Similar to Eq.~\ref{rom:slspg_proj},  a reduced non-linear equation system of dimension $\numSolModes$ can be obtained and viewed as the result of a Petrov-Galerkin projection
\begin{equation}
    (\mathbf{\hat{W}}^\iterIdx)^T \mathbf{P} \mathbf{r}(\mathbf{\tilde{q}}^n_p) = 0,
    \label{rom:lspg_proj}
\end{equation}
where $\mathbf{\hat{W}}$ is the test basis
\begin{equation}
    \mathbf{\hat{W}}^\iterIdx =  \frac{\partial\mathbf{P}\mathbf{r}(\mathbf{\tilde{q}}^n_p)}{\partial\mathbf{\hat{q}}^n_r}.
    \label{rom:lspg_w}
\end{equation}

We point out that two distinct scaling matrices, $\mathbf{P}$ and $\mathbf{H}$, are introduced, so that each equation in FOM equation residual contributes equally to the minimization problem in Eq.~\ref{rom:lspg_def} and the POD bases are appropriately generated, %{\color{red} preserve the conditions of the ROM}
instead of one scaling matrix, $\mathbf{P}$, which is typical for standard model reduction methods (as seen in Section~\ref{StandardROM}).

%\subsubsection{SP-LSVT in physical time form}

We now develop ROMs for the governing equations with transformed solution variables solved via linear multi-step and Runge--Kutta methods.  More detailed derivations of the results below can be found in~\ref{appendix:SP-LSVTTestFunctionPhysicalTime}. 
For linear multi-step methods, the residual in Eq.~\ref{EqRes:LinearMultiStep_qp} yields the test function
\begin{equation}
    \mathbf{\hat{W}}^\iterIdx = \mathbf{P} \left(\hat{\boldsymbol{\Gamma}}^\iterIdx - \dt \beta_0 \hat{\mathbf{J}}^\iterIdx \hat{\boldsymbol{\Gamma}}^\iterIdx \right)\mathbf{H}^{-1}\mathbf{\hat{V}},
    \label{rom:lspg_w_LinearMultistep}
\end{equation}
where $\hat{\mathbf{J}}^\iterIdx = \left[\partial\mathbf{ f }/\partial\mathbf{q}{\color{blue}_p}\right]^\iterIdx_{\mathbf{q}_p=\tilde{\mathbf{q}}_p}$ and $\hat{\boldsymbol{\Gamma}}^\iterIdx = \left[\partial\mathbf{ q }/\partial\mathbf{q}_p\right]^\iterIdx_{\mathbf{q}_p=\tilde{\mathbf{q}}_p}$. It is worthwhile to point out that for an explicit scheme ($\beta_0 = 0$), $\mathbf{\hat{W}}^\iterIdx = \mathbf{P}\hat{\boldsymbol{\Gamma}}^\iterIdx \mathbf{H}^{-1} \mathbf{\hat{V}}$, which is not equivalent to Galerkin projection. %This indicates that under an arbitrary change in solution variables, LSPG projection is not equivalent to Galerkin projection for explicit linear multistep methods. 
Rather, the two projection methods are only equivalent for an explicit integrator when the solution variables are chosen to be the same as that in the semi-discrete form of the equations (i.e. $\mathbf{q}$ for Eq.~\ref{cfd:discretized} and $\mathbf{q}_p$ for Eq.~\ref{cfd:discretized_qp_ge} with $\hat{\boldsymbol{\Gamma}}^\iterIdx = \mathbf{I}$ and $\mathbf{H} = \mathbf{P}$). 

Similarly for Runge--Kutta methods, the equation residual in Eq.~\ref{EqRes:RK_qp} yields the test function
\begin{equation}
    \mathbf{\hat{W}}^\iterIdx = \mathbf{P}\hat{\boldsymbol{\Gamma}}^\iterIdx \mathbf{H}^{-1}\mathbf{\hat{V}},
    \label{rom:lspg_w_RK}
\end{equation}
which is identical to the test function for an explicit linear multi-step time integrator. It should also be pointed out that the test function remains the same for both explicit and implicit Runge--Kutta methods.

For the numerical results presented in the current work,  Newton's method is used to solve Eq.~\ref{rom:lspg_proj}. We derive the iterative procedure for solving SP-LSVT ROMs  to highlight one important property that the method provides -- that is, the symmetrization of the resulting ROM. We introduce a sub-iteration variable $\subIdx$, and define $\mathbf{y}(\mathbf{\hat{q}}^{\subIdx-1}_r) \triangleq(\mathbf{\hat{W}}^{\subIdx-1})^T \mathbf{P} \mathbf{r}(\mathbf{\tilde{q}}^{\subIdx-1}_p)$ for the sake of compactness. Applying Newton's method to Eq.~\ref{rom:lspg_proj} gives

\begin{equation}
    \frac{\partial\mathbf{y}(\mathbf{\hat{q}}^{\subIdx-1}_r)}{\partial\mathbf{\hat{q}}^{\subIdx-1}_r}(\mathbf{\hat{q}}^k_r-\mathbf{\hat{q}}^{\subIdx-1}_r) + \mathbf{y}(\mathbf{\hat{q}}^{\subIdx-1}_r) = 0,
    \label{rom:lspg_proj_newton}
\end{equation}
where 
\begin{equation}
    \frac{\partial\mathbf{y}(\mathbf{\hat{q}}^{\subIdx-1}_r)}{\partial\mathbf{\hat{q}}^{\subIdx-1}_r} = (\mathbf{\hat{W}}^{\subIdx-1})^T \frac{\partial \mathbf{P} \mathbf{r}(\mathbf{\tilde{q}}^{\subIdx-1}_p)}{\partial \mathbf{\hat{q}}^{\subIdx-1}_r} =  (\mathbf{\hat{W}}^{\subIdx-1})^T \mathbf{\hat{W}}^{\subIdx-1}.
    \label{rom:lspg_yJacob}
\end{equation}
Therefore, Eq.~\ref{rom:lspg_proj_newton} can be readily seen as a symmetrized  system. %The importance of this fact will be discussed in  section~\ref{sec:symmetry}. 
Inserting Eq.~\ref{rom:lspg_yJacob} into Eq.~\ref{rom:lspg_proj_newton}, we arrive at the simplified form of Newton's method applied to SP-LSVT ROMs
\begin{equation}
    (\mathbf{\hat{W}}^{\subIdx-1})^T \mathbf{\hat{W}}^{\subIdx-1}(\mathbf{\hat{q}}^k_r-\mathbf{\hat{q}}^{\subIdx-1}_r) + (\mathbf{\hat{W}}^{\subIdx-1})^T \mathbf{P} \mathbf{r} (\mathbf{\tilde{q}}^{\subIdx-1}_p) = 0.
    \label{rom:lspg_proj_newton_symm}
\end{equation}



\subsection{Pseudo-time Stepping}
\label{lspg-vt-pseudo}
To achieve further robustness in simulating highly stiff multi-scale problems, pseudo-time~\cite{sankaranDualTime1995,Pulliam} stepping (or dual time-stepping) can be employed.  %In this section, we derive a strategy to achieve fully discrete symmetrization in SP-LSVT ROM in consistency with FOM on pseudo-time level. 
The pseudo-time ($\tau$) derivative is represented using the implicit Euler method in the following form
 \begin{align}
     \frac{\text{d}\mathbf{q}}{\dPTimeVar}|_{\tau = \tau_k} &= \boldsymbol{\Gamma} \frac{\text{d}\mathbf{q_p}}{\dPTimeVar}|_{\tau = \tau_k} \approx \boldsymbol{\Gamma}^{\subIdx-1} \frac{(\mathbf{q}_p^{\subIdx} - \mathbf{q}_p^{\subIdx-1})}{\Delta\tau},
 \end{align}
 where $\subIdx$ represents the pseudo-time iteration number. During the dual time-stepping procedure, this term is driven to zero. For linear multi-step time integrators, the fully-discrete FOM equation residual with pseudo-time, $\mathbf{r}_p: \mathbb{R}^{\numDOF} \rightarrow \mathbb{R}^{\numDOF}$, takes the form
\begin{align}
\mathbf{r}_p(\mathbf{q}_p^\subIdx) \triangleq & \boldsymbol{\Gamma}^{\subIdx-1} \frac{\dt}{\Delta\tau}(\mathbf{q}_p^{\subIdx} - \mathbf{q}_p^{\subIdx-1}) + \mathbf{r}(\mathbf{q}_p^{\subIdx}) \\
= & \boldsymbol{\Gamma}^{\subIdx-1} \frac{\dt}{\Delta\tau}(\mathbf{q}_p^{\subIdx} - \mathbf{q}_p^{\subIdx-1}) + \mathbf{q}(\mathbf{q}_p^{\subIdx}) + \sum^{\itermaxLinMS}_{j=1}\alpha_j \mathbf{q}(\mathbf{q}_p^{\iterIdx-j}) - \dt \beta_0 \mathbf{f} \left( \mathbf{q}_p^\subIdx, \timeVar^\subIdx\right) - \dt \sum^{\itermaxLinMS}_{j=1} \beta_j\mathbf{f} \left(\mathbf{q}_p^{\iterIdx-j},\timeVar^{\iterIdx-j}\right) %+ \left[\mathbf{q}(\mathbf{q}_p^{\subIdx}) - \mathbf{q}(\mathbf{q}_p^{\subIdx-1})\right] - \dt \beta_0 \left[\mathbf{f} \left(\mathbf{q}_p^\subIdx, \timeVar^\iterIdx\right) - \mathbf{f}\left(\mathbf{q}_p^{\subIdx-1},\timeVar^\iterIdx\right)\right].
\label{EqRes:LinearMultiStep_qp_dualtime}    
\end{align}
Linearizing the second and fourth terms  on the right-hand side
\begin{align}
   \mathbf{q}(\mathbf{q}_p^{\subIdx}) &\approx  \mathbf{q}(\mathbf{q}_p^{\subIdx-1}) +  \left(\frac{\partial\mathbf{q}}{\partial\mathbf{q}_p}\right)^{\subIdx-1}(\mathbf{q}_p^{\subIdx} - \mathbf{q}_p^{\subIdx-1}) = \mathbf{q}(\mathbf{q}_p^{\subIdx-1}) +  \boldsymbol{\Gamma}^{\subIdx-1} (\mathbf{q}_p^{\subIdx} - \mathbf{q}_p^{\subIdx-1}), \\
   %+\sum^{\itermaxLinMS}_{j=1}\alpha_j \mathbf{q}(\mathbf{q}_p^{\subIdx-j}) &\approx \left(\frac{\partial\mathbf{q}}{\partial\mathbf{q}_p}\right)^{\subIdx-1}(\mathbf{q}_p^{\subIdx} - \mathbf{q}_p^{\subIdx-1}) = \boldsymbol{\Gamma}^{\subIdx-1} (\mathbf{q}_p^{\subIdx} - \mathbf{q}_p^{\subIdx-1}), \\
   - \dt \beta_0 \mathbf{f}\left(\mathbf{q}_p^\subIdx,\timeVar^\subIdx\right) &\approx - \dt \beta_0 \mathbf{f}\left(\mathbf{q}_p^{\subIdx-1},\timeVar^{\subIdx-1}\right) - \dt \beta_0 \mathbf{J}^{\subIdx-1}\boldsymbol{\Gamma}^{\subIdx-1}(\mathbf{q}_p^{\subIdx} - \mathbf{q}_p^{\subIdx-1}),
%= & - \Delta \text{t} \beta_0 \left(\frac{\partial\mathbf{f}}{\partial\mathbf{q}}\right)^{k-1}\left(\frac{\partial\mathbf{q}}{\partial\mathbf{q_p}}\right)^{k-1}(\mathbf{q}_p^{k} - \mathbf{q}_p^{k-1}) \\
%- \dt \beta_0\left[\mathbf{f}\left(\mathbf{q}_p^\subIdx,\timeVar^\iterIdx\right) - \mathbf{f}\left(\mathbf{q}_p^{\subIdx-1},\timeVar^\iterIdx\right)\right] &\approx %- \Delta \text{t} \beta_0 \left(\frac{\partial\mathbf{f}}{\partial\mathbf{q}_p}\right)^{k-1}(\mathbf{q}_p^{k} - \mathbf{q}_p^{k-1}) \\
%= & - \Delta \text{t} \beta_0 \left(\frac{\partial\mathbf{f}}{\partial\mathbf{q}}\right)^{k-1}\left(\frac{\partial\mathbf{q}}{\partial\mathbf{q_p}}\right)^{k-1}(\mathbf{q}_p^{k} - \mathbf{q}_p^{k-1}) \\
%= & 
%- \dt \beta_0 \mathbf{J}^{\subIdx-1}\boldsymbol{\Gamma}^{\subIdx-1}(\mathbf{q}_p^{\subIdx} - \mathbf{q}_p^{\subIdx-1}),
\end{align}
and collecting terms, the final form of Eq.~\ref{EqRes:LinearMultiStep_qp_dualtime} becomes
\begin{equation}
    \mathbf{r}_p(\mathbf{q}_p^\subIdx) = \left[\left(\frac{\dt}{\Delta\tau} + 1\right) \boldsymbol{\Gamma}^{\subIdx-1} - \dt \beta_0 \mathbf{J}^{\subIdx-1}\boldsymbol{\Gamma}^{\subIdx-1}  \right] (\mathbf{q}_p^{\subIdx} - \mathbf{q}_p^{\subIdx-1})+\mathbf{r}(\mathbf{q}_p^{\subIdx-1}).
    \label{EqRes:LinearMultiStep_qp_DualTime}
\end{equation}
If $\beta_0 = 0$, the time integration formulation is explicit; otherwise, it is implicit. 

Following the same procedure, the fully-consistent discrete FOM equation residual for Runge--Kutta methods becomes
\begin{equation}
    \mathbf{r}_p(\mathbf{q}_p^\subIdx) = \left[\left(\frac{\dt}{\Delta\tau} + 1\right) \boldsymbol{\Gamma}^{\subIdx-1} \right]  (\mathbf{q}_p^{\subIdx} - \mathbf{q}_p^{\subIdx-1})+\mathbf{r}(\mathbf{q}_p^{\subIdx-1}).
    \label{EqRes:RK_qp_dualtime}
\end{equation}

With sufficient convergence, $\mathbf{r}_p (\mathbf{q}^{\subIdx}_p) \rightarrow \mathbf{0}$ and $(\mathbf{q}^{\subIdx}_p - \mathbf{q}^{\subIdx-1}_p) \rightarrow \mathbf{0}$. Thus, the fully-discrete FOM residual is also driven to zero (i.e. $\mathbf{r}(\mathbf{q}^{\subIdx}_p) \rightarrow \mathbf{0}$), achieving consistency with the conservative formulation. At this point, the solution is advanced in physical time, $\mathbf{q}^{\iterIdx}_p = \mathbf{q}^{\subIdx-1}_p$.

Therefore, if a dual-time algorithm is used  to solve Eq.~\ref{rom:lspg_proj} instead of Newton's method in Eq.~\ref{rom:lspg_proj_newton_symm}, the SP-LSVT ROM formulation applied to the physical time residual becomes
\begin{equation}
    (\mathbf{\hat{W}}^\subIdx)^T \left[ \left(\frac{\dt}{\Delta\tau}\hat{\boldsymbol{\Gamma}}^{\subIdx-1} + \mathbf{\hat{W}}^\subIdx\right) (\mathbf{\hat{q}}^k_r - \mathbf{\hat{q}}^{\subIdx-1}_r) + \mathbf{r}(\mathbf{\tilde{q}}^{\subIdx-1}_p) \right] = 0.
    \label{rom:lspg_proj_dualtime_nonsymmetric}
\end{equation}
It can be easily recognized that when $\Delta \tau \rightarrow \infty$, we recover the Newton's method form (Eq.~\ref{rom:lspg_proj_newton_symm}). For finite $\Delta \tau$, however, the above equation is not symmetrized at the sub-iteration level. This issue is addressed in the following discussion.

\subsection{Discrete Consistency and Symmetrization}
\label{lspg-vt-dualtime}

%Next, we derive a  formulation for the SP-LSVT ROM method using the pseudo-time formulation (Eq.~\ref{EqRes:RK_qp_dualtime}). 
We now reformulate the objective to minimize the fully-discrete FOM equation residual at the sub-iteration (or pseudo-time step) level. In this context, Eqs.~\ref{EqRes:LinearMultiStep_qp_DualTime} and~\ref{EqRes:RK_qp_dualtime} are minimized with respect to $\mathbf{\tilde{q}}^{\subIdx}_p = \mathbf{q}_{p,\text{ref}} + \mathbf{H}^{-1}\mathbf{\hat{V}}\mathbf{\hat{q}}^{\subIdx}_r$. Therefore, we define
\begin{equation}
     \tilde{\mathbf{q}}^k_p  \triangleq  \arg \min_{ \tilde{\mathbf{q}}^k_p  \in \textrm{Range}(\mathbf{\hat{V}})} \norm{\mathbf{P}\mathbf{r}_p(\mathbf{\tilde{q}}^k_p)}^2,
    \label{rom:lspg_def_dualtime}
\end{equation}
with the equation residual, $\mathbf{r}$, scaled by matrix, $\mathbf{P}$. Again, the solution to Eq.~\ref{rom:lspg_def_dualtime} %via the Gauss-Newton method 
has an equivalent semi-discrete Petrov-Galerkin projection form given by
\begin{equation}
    (\mathbf{\tilde{W}}^\subIdx)^T \mathbf{P} \mathbf{r}_p(\mathbf{\tilde{q}}^k_p) = 0,
    \label{rom:lspg_proj_dualtime}
\end{equation}
where $\mathbf{\tilde{W}}$ is the test basis
\begin{equation}
    \mathbf{\tilde{W}}^\subIdx = \frac{\partial\mathbf{P}\mathbf{r}_p(\mathbf{\tilde{q}}^k_p)}{\partial\mathbf{\hat{q}}^k_r}.
\end{equation}

For linear multi-step methods, the FOM equation residual $\mathbf{r}_p$ is defined in Eqs.~\ref{EqRes:LinearMultiStep_qp_DualTime}. Substituting the approximate solutions, $\mathbf{\tilde{q}}^k_p$ and $\mathbf{\tilde{q}}^{\subIdx-1}_p$, we have %arrives at
%\begin{equation}
   % \mathbf{r}_p(\mathbf{\tilde{q}}_p^\subIdx) = \left[\left(\frac{\dt}{\Delta\tau} + 1\right) \hat{\boldsymbol{\Gamma}}^{\subIdx-1} - \dt \beta_0 \hat{\mathbf{J}}^{\subIdx-1}\hat{\boldsymbol{\Gamma}}^{\subIdx-1}  \right]  (\mathbf{\tilde{q}}_p^{\subIdx} - \mathbf{\tilde{q}}_p^{\subIdx-1})+\mathbf{r}(\mathbf{\tilde{q}}_p^{\subIdx-1}).
    \label{RomRes:LinearMultiStep_qp_DualTime}
%\end{equation}
%Therefore
\begin{equation}
    \frac{\partial\mathbf{P}\mathbf{r}_p(\mathbf{\tilde{q}}^k_p)}{\partial\mathbf{\hat{q}}^k_r} = \frac{\partial\mathbf{P}\mathbf{r}_p(\mathbf{\tilde{q}}^k_p)}{\partial\mathbf{\tilde{q}}^k_p}\frac{\partial\mathbf{\tilde{q}}^k_p}{\partial\mathbf{\hat{q}}^k_r} = \mathbf{P}\left[\left(\frac{\dt}{\Delta\tau} + 1\right) \hat{\boldsymbol{\Gamma}}^{\subIdx-1} - \dt \beta_0 \hat{\mathbf{J}}^{\subIdx-1}\hat{\boldsymbol{\Gamma}}^{\subIdx-1} \right] \mathbf{H}^{-1} \mathbf{\hat{V}}.
\end{equation}
Hence, the test basis $\mathbf{\tilde{W}}^\subIdx$ becomes
\begin{equation}
    \mathbf{\tilde{W}}^\subIdx = \mathbf{P}\left[\left(\frac{\dt}{\Delta\tau} + 1\right) \hat{\boldsymbol{\Gamma}}^{\subIdx-1} - \dt \beta_0 \hat{\mathbf{J}}^{\subIdx-1}\hat{\boldsymbol{\Gamma}}^{\subIdx-1} \right] \mathbf{H}^{-1} \mathbf{\hat{V}}.
    \label{rom:lspg_w_qp_DualTime}
\end{equation}

Similarly, we can derive the discretely-consistent SP-LSVT ROM formulation for Runge--Kutta methods. The FOM equation residual is defined in Eq.~\ref{EqRes:RK_qp_dualtime}. Again substituting the approximate solutions, $\mathbf{\tilde{q}}^k_p$ and $\mathbf{\tilde{q}}^{\subIdx-1}_p $, results in the ROM residual

\begin{equation}
    \mathbf{r}_p(\mathbf{\tilde{q}}_p^\subIdx) = \left[\left(\frac{\dt}{\Delta\tau} + 1\right) \hat{\boldsymbol{\Gamma}}^{\subIdx-1} \right]  (\mathbf{\tilde{q}}_p^{\subIdx} - \mathbf{\tilde{q}}_p^{\subIdx-1})+\mathbf{r}(\mathbf{\tilde{q}}_p^{\subIdx-1}).
\end{equation}
Therefore
\begin{equation}
    \frac{\partial\mathbf{P}\mathbf{r}_p(\mathbf{\tilde{q}}^k_p)}{\partial\mathbf{\hat{q}}^k_r} = \frac{\partial\mathbf{P}\mathbf{r}_p(\mathbf{\tilde{q}}^k_p)}{\partial\mathbf{\tilde{q}}^k_p}\frac{\partial\mathbf{\tilde{q}}^k_p}{\partial\mathbf{\hat{q}}^k_r} = \mathbf{P}\left[\left(\frac{\dt}{\Delta\tau} + 1\right) \hat{\boldsymbol{\Gamma}}^{\subIdx-1} \right] \mathbf{H}^{-1} \mathbf{\hat{V}}.
\end{equation}
Hence, the test basis $\mathbf{\tilde{W}}^\subIdx$ becomes
\begin{equation}
    \mathbf{\tilde{W}}^\subIdx = \mathbf{P}\left[\left(\frac{\dt}{\Delta\tau} + 1\right) \hat{\boldsymbol{\Gamma}}^{\subIdx-1} \right] \mathbf{H}^{-1} \mathbf{\hat{V}}.
    \label{rom:lspg_w_qp_DualTime_rk}
\end{equation}

It can be readily seen that SP-LSVT ROMs using either linear multi-step and Runge--Kutta methods lead to the symmetrized formulation
\begin{equation}
    (\mathbf{\tilde{W}}^\subIdx)^T \left[\mathbf{\tilde{W}}^\subIdx (\mathbf{\hat{q}}^k_r - \mathbf{\hat{q}}^{\subIdx-1}_r) + \mathbf{r}(\mathbf{\tilde{q}}^{\subIdx-1}_p) \right] = 0.
    \label{rom:lspg_proj_dualtime_symmetric_rk}
\end{equation}


\subsection{A Note on Symmetrization}
\label{sec:symmetry}
The benefits of symmetrization have been examined in  many contexts in the literature. For instance, Ref.~\cite{SymmetrizedODE} discusses applications in ODE systems.  Barone et al.~\cite{Barone2009JCP} have shown that symmetrization   provides enhanced stabilization and convergence of the discrete ROM system. In our context, symmetrization guarantees linear stability of the ROMs, subject to linear stability restrictions on the FOM, as shown in Section~\ref{proof}.

As shown in Eq.~\ref{rom:lspg_proj_newton_symm}, a symmetrized discrete system can also be obtained if the SP-LSVT ROM formulation is applied to fully-discrete equation residual in physical time (Eq.~\ref{rom:lspg_def}) and Newton's method is used to solve the reduced system. We also demonstrated (Eq.~\ref{rom:lspg_proj_dualtime_nonsymmetric}) that, if a dual-time algorithm is used, the SP-LSVT ROM formulation applied to the physical time residual results in a unsymmetrized ROM system.
%\begin{equation}
%    (\mathbf{\hat{W}}^k)^T \left[ %\left(\frac{\boldsymbol{\Gamma}^{k-1}}{\Delta\tau} + %\mathbf{\hat{W}}^k\right) (\mathbf{\hat{q}}^k_r - \mathbf{\hat{q}}^{k-1}_r) %+ \mathbf{r}(\mathbf{\hat{V}}\mathbf{\hat{q}}^{k-1}_r) \right] = 0.
%    \label{rom:lspg_proj_dualtime_nonsymmetric}
%\end{equation}
Therefore, to ensure symmetrization while using dual time-stepping, the SP-LSVT ROM must be formulated for the pseudo-time residual as given by Eq.~\ref{rom:lspg_proj_dualtime_symmetric_rk}.


%The LSPG projection method proposed by Carlberg et al.~\cite{Carlberg2017} requires implicit time integration, as applying the LSPG projection with explicit time integration is equivalent to Galerkin projection. However, in this work, 


In summary, we have shown that with a more general selection of solution variables, symmetrized least-squares-based Petrov-Galerkin projections can be derived at the fully discrete sub-iteration level.  These formulations are also applicable to systems discretized with explicit time integrators. In Section~\ref{results}, we will assess the robustness and accuracy of ROMs using Galerkin projection, LSPG projection, and the SP-LSVT ROM formulation for challenging reacting flow problems.

==> figures/Limiters.tex <==
\section{Enhancing Local Stability}
\label{limiters}
While symmetrization improves the prospects for global stability, ROMs of complex problems can fail because of spurious local behavior.  The current authors~\cite{HuangAIAAJ2019,Huang2020_SpeciesLimiters} have demonstrated that imposing physical realizability during ROM calculations can be critical to ROM stability. This is especially important when the trial basis is not rich enough to resolve sharp gradients in the flow field, resulting in spurious oscillations. In reacting flows, this often leads to unrealistic values of physical quantities (e.g. $T \leq 0$ K), terminating the calculations. 
The SP-LSVT ROM formulation cannot guarantee positivity of quantities such as density or temperature. Therefore, to mitigate the production of such spurious oscillations near sharp gradients, local limiters can be deployed. 


In the rocket combustion ROMs presented in this work, two types of simple limiters are proposed: one for temperature and the other for species mass fractions. The temperature limiter follows the method proposed by the current authors~\cite{HuangAIAAJ2019} to restrict the temperature $\Tilde{T}$ in ROM calculations (based on Eq.~\ref{pod:expansion_qp})  %$\Tilde{T} = T_{ref} + \mathbf{H}^{-1}_{T}\mathbf{\hat{V}}_{T} \mathbf{\hat{q}}_r$ 
to an interval bounded by  $T_{min}$,  $T_{max}$. This range can be determined based on the underlying physics. In non-premixed flames, for example, physics dictates that the minimum and maximum temperatures in the simulation are bounded by the cold reactant temperature, $T_{c}$, and the adiabatic flame temperature, $T_{ad}$, respectively. This range can be can be determined \textit{a priori} based on the propellants and flow configuration  before running the FOM simulations. For example, $T_{min} = T_{c} - \delta T_c$ and $T_{min} = T_{ad} + \delta T_{ad}$, where values of $\delta T_c$ and $\delta T_{ad}$ can be estimated to account for temperature variations due to the effects of acoustics and thermodynamics. 

In contrast to  spurious oscillations in temperature which can terminate the ROM calculations immediately, the generation of spurious oscillations in the species mass fraction fields exhibits a more gradual  impact on the ROM results, as diagnosed in previous work~\cite{Huang2020_SpeciesLimiters}. This can be particularly problematic within the high temperature reaction regions. As a demonstrative example, a 1D premixed flame is considered in~\ref{appendix:species_oscillations}. To suppress these spurious oscillations in reaction regions, limiters on species mass fraction fields (denoted as the \emph{species limiter} in the rest of the paper for simplicity) are proposed for premixed and non-premixed flames. 

For a \emph{premixed} flame
\begin{equation}
    \text{if} \; \Tilde{T} > T_{th}, \; \Tilde{Y}_{R} = min \{ \Tilde{Y}_{R}, \delta \},
    \label{rom:species_limiter_premixed}
\end{equation}
The limiter is only activated in the reacting regions when  $\Tilde{T}$ exceeds a certain threshold value $T_{th}$, which can be predetermined based on the adiabatic flame temperature, $T_{ad}$ (e.g. $T_{th} = 0.8 T_{ad}$). $\Tilde{Y}_{R}$ represents the mass fraction of reactants in ROM calculations and $\delta$ is a small value (e.g. $1 \times 10^{-5}$).

Similarly, for a \emph{non-premixed} flame, the limiter is only activated in the reacting regions
\begin{equation}
    \text{if} \; \Tilde{T} > T_{th}, \left\{\begin{array}{lll}
        \text{if} \; \Tilde{Z} > Z_{st}, & \Tilde{Y}_{ox} & = min \{ \Tilde{Y}_{ox}, \delta \} \\
        \text{if} \; \Tilde{Z} = Z_{st}, & \Tilde{Y}_{f} & = min \{ \Tilde{Y}_{f}, \delta \} \;\; \text{and} \;\; \Tilde{Y}_{ox} = min \{ \Tilde{Y}_{ox}, \delta \} \\
        \text{if} \; \Tilde{Z} < Z_{st}, & \Tilde{Y}_{f} & = min \{ \Tilde{Y}_{f}, \delta \}
    \end{array} \right .
    \label{rom:species_limiter_nonpremixed}
\end{equation}
where $\Tilde{Z}$ is the mixture fraction
\begin{equation}
\Tilde{Z} = \frac{ \nu_{st} \Tilde{Y}_f - \Tilde{Y}_{ox} + Y^0_{ox} }{ \nu_{st} Y^0_{f} + Y^0_{ox} }.
\label{mixture_fraction}
\end{equation}
Here, $\nu_{st}$ is the stoichiometric oxidizer-to-fuel mass fraction ratio, $\Tilde{Y}_f$ and $\Tilde{Y}_{ox}$ are the fuel and oxidizer mass fractions respectively, and $Y^0_f$ and $Y^0_{ox}$ are the mass fraction of fuel and oxidizer in the fuel and oxidizer inlet streams, respectively. The constant parameters $\nu_{st}$ , $Y^0_f$ and $Y^0_{ox}$ can be predetermined based on the reacting flow propellants and conditions before running the FOM simulations. $Z_{st}$ is the stoichiometric mixture fraction, $Z_{st} = Y^0_{ox} / ( \nu_{st} Y^0_{f} + Y^0_{ox} )$. As indicated in Eq.~\ref{rom:species_limiter_nonpremixed}, only the mass fraction of oxidizer, $\Tilde{Y}_{ox}$ is limited in fuel-rich reaction regions ($\Tilde{Z} > Z_{st}$). In fuel-lean reaction regions ($\Tilde{Z} < Z_{st}$), only the mass fraction of fuel, $\Tilde{Y}_f$, is limited. In stoichiometric reaction regions ($\Tilde{Z} = Z_{st}$), both are limited. 

Note that the species limiter in Eqs.~\ref{rom:species_limiter_premixed} and~\ref{rom:species_limiter_nonpremixed} is designated for chemical reactions modeled by multi-species transport equations. For a flamelet-type model~\cite{Pierce2004_FPV} where chemical reactions are modeled by representative transported scalars (e.g. mixture fraction $Z$ and progress variable $C$), the species limiter for a \emph{premixed} flame becomes
\begin{equation}
    \text{if} \; \Tilde{T} > T_{th}, \; \Tilde{C} = min \{max \{ \Tilde{C}, C_\text{ref} - \delta \}, C_\text{ref} + \delta \},
    \label{rom:species_limiter_flpremixed}
\end{equation}
where $\tilde{C}$ is the progress variable in ROM calculations that represents the progress of the chemical reaction and $C_\text{ref}$ is the highest progress variable value in the problem of interest (e.g. for a stoichiometric reaction, $C_\text{ref}=1$, while for non-stoichiometric reaction, $C_\text{ref}<1$). 

Similarly, for a \emph{non-premixed} flame, the limiter becomes
\begin{equation}
    \text{if} \; \Tilde{T} > T_{th}, \left\{\begin{array}{ll}
        \Tilde{C} = min\{max \{ \Tilde{C}, C_\text{ref} - \delta \}, C_\text{ref} + \delta \} \\
        \Tilde{Z} = min \{ max \{ \Tilde{Z}, Z_{st} - \delta\}, Z_{st} + \delta \}
    \end{array} \right .
    \label{rom:species_limiter_flnonpremixed}
\end{equation}
where both the progress variables $\Tilde{C}$ and mixture fraction $\Tilde{Z}$ in ROM calculations need to be limited. The benefits of imposing the species limiter is further demonstrated using a 2D non-premixed reacting flow problem in Sec.~\ref{sec:2d_limiters}.

The above discussion emphasizes the importance of local robustness considerations in ROMs of complex problems. 

==> figures/Proofs.tex <==
\section{Stability
of Least-Squares-based ROMs for Linear Problems}
\label{proof}
In this section, we provide a complete proof of least-squares-based ROMs for a linear time-invariant (LTI) system. While the finite element community is rich with literature on the analysis of least-squares-based techniques (e.g. ~\cite{LSFEM}), rather surprisingly, we have not found a stability analysis in the ROM literature. We pursue a linear algebra standpoint, which will be useful for the analysis of numerical results in Section~\ref{2d:LinearStability}.

For the full order model, we assume an autonomous LTI system given by
\begin{equation}
    \frac{\text{d}\mathbf{q}}{\dTimeVar}=\mathbf{J}\mathbf{q}, \ \ \mathbf{q}(0) = \mathbf{q}_0,
    \label{LTI}
\end{equation}
where $\mathbf{q} \in {\mathbb{R}^{\numDOF}}$, and $\mathbf{J} \in \mathbb{R}^{\numDOF \times \numDOF}$. 
For clarity of presentation, we will consider a backward Euler discretization for the FOM:
\begin{align}
  \mathbf{q}^n  &= (\mb{I} - \Delta t \mb{J})^{-1} \mathbf{q}^{n-1}, \ \  \mathbf{q}^0 = \st{\mathbf{V}\mathbf{V}^T} \mathbf{q}_0.
    \label{LTI:discrete}
\end{align}

Consider a low-rank representation $\mathbf{\tilde{q}}(\timeVar) \triangleq \mathbf{V}\mathbf{q}_r(\timeVar)$, where $\mb{V} \in \mathbb{R}^{\numDOF \times k}$ and $\mb{q}_r \in \mathbb{R}^k$. Note: The main conclusions also hold when $\mathbf{\tilde{q}}(\timeVar) \triangleq \mb{q}_{ref} + \mb{P}^{-1} \mathbf{V}\mathbf{q}_r(\timeVar)$.

\subsection{Least-Squares Petrov Galerkin ROM}
Following the development in Section~\ref{slspg_rom}, we get
\begin{equation}
\mb{W}^T \frac{ \tilde{\mb{q}}^n - \tilde{\mb{q}}^{n-1} }{\Delta t} =  \mb{W}^T \mb{J} \tilde{\mb{q}}^n,
\label{LTI:ROMT}
\end{equation}
where $\mb{W} \triangleq (\mb{I}-\Delta t \mb{J})\mb{V}.$ Manipulating further, we get the governing equations for the modal coefficients in the form
\begin{equation}
(\mb{W}^T \mb{W}) \mb{q}_r^n =  \mb{W}^T \mb{V} \mb{q}_r^{n-1}, \ \ \mathbf{q}_r^0 = \mb{V}^T \mathbf{q}_0.
\label{LTI:ROM}
\end{equation}
 We will now prove the stability of the ROM (Eq.~\ref{LTI:ROM}) under the condition that the FOM (Eq.~\ref{LTI:discrete}) is linearly stable. 

We will pursue a notion of stability via the Euclidean vector-induced matrix norm $\norm{\cdot}.$ We will use $\sigma_i(\mb{A})$ to represent the $i^{th}$ singular value of a matrix $\mb{A}$. For a real symmetric matrix $\mb{S}$, we will use $\lambda_j(\mb{S})$ to represent the $j^{th}$ eigenvalue of $\mb{S}$, with the eigenvalues arranged in descending order.

\vspace{0.75cm}

\noindent{\bf Theorem 1} : If the FOM given by Equation~\ref{LTI:discrete} is asymptotically stable in the sense of $\norm{(\mb{I} - \Delta t \mb{J})^{-1}} \leq 1$, then the ROM given by Equation~\ref{LTI:ROM} is also asymptotically stable with no further assumptions required.
\vspace{0.25cm}
\noindent {\em Proof}:
The problem statement reduces to showing that
 $$\norm{(\mb{W}^T \mb{W})^{-1} \mb{W}^T \mb{V}}  \leq 1,$$
 with $\mb{W}\triangleq \mb{B}\mb{V}$, where $\mb{B} \triangleq \mb{I}-\Delta t \mb{J}$, given $\norm{\mb{B}^{-1}} \leq 1.$

Since $\mb{B}$ and $\mb{V}$ are both full-rank matrices, $\mb{W}$ is also a full-rank matrix, and the left pseudo-inverse $\mb{W}^+ \triangleq (\mb{W}^T \mb{W})^{-1} \mb{W}^T$ also exists. Therefore, given $\norm{\mb{W}^+}= \frac{1}{\sigma_k(\mb{W})}$ we have 
\begin{equation}
 \norm{(\mb{W}^T \mb{W})^{-1} \mb{W}^T \mb{V}} = \norm{\mb{W}^+   \mb{V}} \leq  \norm{\mb{W}^+} \norm{\mb{V}}
 = \frac{1}{\sigma_k(\mb{W})}
 \label{eq:proof}
\end{equation}
and thus our problem reduces to showing 

\begin{equation}
    \sigma_k(\mb{W}) = \sigma_k(\mb{B}\mb{V}) \geq 1, \ \ \textrm{given} \ \ \sigma_n(\mb{B}) \geq 1.
    \label{eq:neweq}
\end{equation}


We write $\mb{W}^T \mb{W} = \mb{V}^T \mb{B}^T \mb{B} \mb{V}$
and use the Poincare separation theorem (~\ref{appendix:poincare})  which yields
$$
\lambda_{k}(\mb{W}^T \mb{W}) \geq \lambda_{n} (\mb{B}^T \mb{B}).
$$
Since $\lambda_{k}(\mb{W}^T \mb{W}) = \sigma_k(\mb{W})$ and  $\lambda_{n}(\mb{B}^T \mb{B}) = \sigma_n(\mb{B})$, we have
$$
\sigma_{k}(\mb{W}) \geq \sigma_{n} (\mb{B}).
$$
Since $ \sigma_{n} (\mb{B}) \geq 1$, we have $\sigma_{k}(\mb{W}) \geq 1$. This completes the proof following Equation~\ref{eq:proof}. 

\vspace{0.75cm}

\st{\noindent Note: Galerkin projection on the above problem yields}
\st{\begin{equation}
\mb{V}^T \frac{ \tilde{\mb{q}}^n - \tilde{\mb{q}}^{n-1} }{\Delta t} =  \mb{V}^T \mb{J} \tilde{\mb{q}}^n,
\label{LTI:ROMTG}
\end{equation}
which yields}
\subsection{{\color{blue} Galerkin ROMs}}
{\color{blue} Galerkin projection  on Eq.~\ref{LTI:discrete} yields}
\begin{equation}
(\mb{I}-\Delta t \mb{V}^T \mb{J}\mb{V})\mb{q}_r^n =   \mb{q}_r^{n-1}.
\label{LTI:ROMG}
\end{equation}
Stability demands $\norm{(\mb{I}-\Delta t \mb{V}^T \mb{J} \mb{V})^{-1}} \leq 1$. This can be written as $\norm{(\mb{V}^T \mb{B} \mb{V})^{-1}} \leq 1$, with $\mb{B} \triangleq \mb{I}-\Delta t \mb{J}$. 

$\bullet$ If $\mb{J}$ is a symmetric matrix, $\norm{(\mb{V}^T \mb{B} \mb{V})^{-1}} = \frac{1}{\lambda_k(\mb{V}^T \mb{B} \mb{V})}$. Also note that $\mb{J}$ is negative definite, $\mb{B}$ will be positive definite. Thus, we have $$\lambda_k(\mb{V}^T \mb{B} \mb{V}) \geq \lambda_n(\mb{B}) \geq 1,$$ where the first inequality is due to the Poincare separation theorem, and the second one is due to the fact that $\mb{J}$ is negative-definite. Thus, given that the FOM is asymptotically stable, the Galerkin ROM is asymptotically stable with no further assumptions required.

$\bullet$ If $\mb{J}$ is not a symmetric matrix, then $\norm{(\mb{V}^T \mb{B} \mb{V})^{-1}} = \frac{1}{\sigma_k(\mb{V}^T \mb{B} \mb{V})}$ and thus we have to show that $\sigma_k(\mb{V}^T \mb{B} \mb{V}) \ge 1$. While a convenient upper bound exists (refer~\ref{appendix:poincare}) $\sigma_k(\mb{V}^T \mb{B} \mb{V}) \leq \sigma_k(\mb{B})$,  tight lower bounds do not exist for general non-symmetric $\mb{B}$. Thus unconditional stability (or instability) cannot be proven, and a case-by-case approach is required, depending on the structure of $\mb{J}$ and the time-step $\Delta t$.  It should, however, be noted that, even when the FOM represents a discretization of Hyperbolic PDEs, the underlying numerical dissipation in the FOM, coupled with a small time-step $\Delta t$ can stabilize Galerkin ROMs depending on the level of mode truncation.


\vspace{0.75cm}
{\color{blue}
\noindent{\bf Theorem 2} : If the FOM given by Equation~\ref{LTI:discrete} is asymptotically stable in the sense of $\norm{(\mb{I} - \Delta t \mb{J})^{-1}} \leq 1$, then the Galerkin ROM given by Equation~\ref{LTI:ROMG} is also asymptotically stable if $\lambda_{n}\left( \mb{I}-0.5 \Delta t (\mb{J}+\mb{J}^T)\right) \geq 1.$



\vspace{0.25cm}
\noindent {\em Proof:} Define $\mb{B} \triangleq \mb{I}-\Delta t \mb{J}$. The goal is to show $\sigma_k(\mb{V}^T\mb{B}\mb{V}) \geq 1.$

From Appendix A.3, 
$$ \sigma_i(\mb{V}^T \mb{B} \mb{V}) \geq \lambda_i \left(\mb{V}^T \frac{\mb{B}+\mb{B}^T}{2} \mb{V}  \right) $$

From Appendix A.1, 
$$  \lambda_i \left(\mb{V}^T \frac{\mb{B}+\mb{B}^T}{2} \mb{V}  \right) \geq \lambda_{n-k+i}\left( \frac{\mb{B}+\mb{B}^T}{2}\right).$$

Therefore
$$\sigma_k(\mb{V}^T \mb{B} \mb{V}) \geq \lambda_n\left( \frac{\mb{B}+\mb{B}^T}{2}\right)$$ and stability demands
$$ \lambda_n\left( \frac{\mb{B}+\mb{B}^T}{2}\right) \geq 1.$$
\vspace{0.75cm}

\noindent Note: It can be easily verified, for instance, that a Galerkin ROM of a linear upwind spatial discretization of the linear advection equation with Euler implicit time integration is unconditionally stable. 

}
%\begin{comment}
%\noindent Note: The above condition is not too restrictive.
%Consider $$\frac{\partial u}{\partial t}+a \frac{\partial u}{\partial x}=0.$$
%Defining $\nu \triangleq a \frac{\Delta t}{\Delta x}$, Euler Implicit with first order upwind yields
%$$\mb{B} = \mb{T}[-\nu,1+\nu,0], $$ where $\mb{T}$ represents a tridiagonal matrix with lower diagonal $-\nu,$ diagonal $1+\nu$ and upper diagonal element $0.$ In the periodic case, $\lambda_n\left( \frac{\mb{B}+\mb{B}^T}{2}\right) = 1.$ In the non-periodic case, $\lambda_n\left( \frac{\mb{B}+\mb{B}^T}{2}\right) = 1+\nu \epsilon$, where $\epsilon > 0 $ is related to the mesh resolution. The Galerkin ROM is unconditionally stable in both cases.

%\noindent Note: Galerkin projection on the above problem yields
%\begin{equation}
%\mb{V}^T \frac{ \tilde{\mb{q}}^n - \tilde{\mb{q}}^{n-1} }{\Delta t} =  %\mb{V}^T \mb{J} \tilde{\mb{q}}^n,
%\label{LTI:ROMTG}
%\end{equation}
%which yields 
%\begin{equation}
%(\mb{I}-\Delta t \mb{V}^T \mb{J}\mb{V})\mb{q}_r^n =   \mb{q}_r^{n-1}.
%\label{LTI:ROMG}
%\end{equation}
%Stability demands $\norm{(\mb{I}-\Delta t \mb{V}^T \mb{J} \mb{V})^{-1}} \leq 1$. This can be written as $\norm{(\mb{V}^T \mb{B} \mb{V})^{-1}} \leq 1$, with $\mb{B} \triangleq \mb{I}-\Delta t \mb{J}$. 

%$\bullet$ If $\mb{J}$ is a symmetric matrix, $\norm{(\mb{V}^T \mb{B} \mb{V})^{-1}} = \frac{1}{\lambda_k(\mb{V}^T \mb{B} \mb{V})}$. Also note that $\mb{J}$ is negative definite, $\mb{B}$ will be positive definite. Thus, we have $$\lambda_k(\mb{V}^T \mb{B} \mb{V}) \geq \lambda_n(\mb{B}) \geq 1,$$ where the first inequality is due to the Poincare separation theorem, and the second one is due to the fact that $\mb{J}$ is negative-definite. Thus, given that the FOM is asymptotically stable, the Galerkin ROM is asymptotically stable with no further assumptions required.

%$\bullet$ If $\mb{J}$ is not a symmetric matrix, then $\norm{(\mb{V}^T \mb{B} \mb{V})^{-1}} = \frac{1}{\sigma_k(\mb{V}^T \mb{B} \mb{V})}$ and thus we have to show that $\sigma_k(\mb{V}^T \mb{B} \mb{V}) \ge 1$. While a convenient upper bound exists (refer~\ref{appendix:poincare}) $\sigma_k(\mb{V}^T \mb{B} \mb{V}) \leq \sigma_k(\mb{B})$,  tight lower bounds do not exist for general non-symmetric $\mb{B}$. Thus unconditional stability (or instability) cannot be proven, and a case-by-case approach is required, depending on the structure of $\mb{J}$ and the time-step $\Delta t$.  It should, however, be noted that, even when the FOM represents a discretization of Hyperbolic PDEs, the underlying numerical dissipation in the FOM, coupled with a small time-step $\Delta t$ can stabilize Galerkin ROMs depending on the level of mode truncation.


%\begin{comment}
%We prove such a result below.

%\vspace{0.75cm}
%\noindent{\bf Theorem 2} : If the time step $\Delta t$ is chosen such that $ \norm{\Delta t \mb{J}} \leq \alpha$, then the Galerkin ROM given by Equation~\ref{LTI:ROMG} is asymptotically stable in the sense of $\norm{(\mb{I} - \Delta t \mb{V}^T \mb{J} \mb{V})^{-1}} \leq 1$ with no further assumptions required.
%\vspace{0.25cm}
%\noindent {\em Proof:} Since $\norm{\Delta t \mb{J}} \le 1,$ we have $\sigma_1(\Delta t \mb{V}^T  \mb{J} \mb{V}) \leq \sigma_1(\Delta t \mb{J})$. This inequality is because of a singular value transformation identity (refer~\ref{appendix:poincare}). Since $\sigma_1(\Delta t \mb{V}^T  \mb{J} \mb{V}) < 1$, we have $\norm{} < 1$
%\vspace{0.75cm}

%\end{comment}

%\end{comment}

%\clearpage Thus, for non-symmetric $\mb{B}$, the Galerkin method may be stable or unstable on a case-by-case basis. It is not necessary that a Galerkin ROM developed from discretizations of Hyperbolic PDEs would be unstable, because the dissipation terms present in the FOM can stabilize the ROM.

==> figures/Reviewer1.tex <==
\noindent \textbf{Reviewer 1's comments}

In the manuscript, the authors presented a least-squares projection based ROM method for
complex multi-scale problems, in particular the rocket combustion. It is very convenient to have
the freedom of choosing solution variables in constructing ROMs of compressible flows, which is guaranteed by a transformation in this manuscript. The symmetrization of the ROM scheme is obtained by a consistent computation of Jacobian in implicit time stepping. Local stability is also enhanced by bounding the temperature and using species limiter. The numerical results for 2D and 3D rocket comustion are convincing. I can recommend publication of this paper in JCP, provided that the following concerns are addressed.

\begin{enumerate}

\item The authors claimed that SP-LSVT is structure-preserving. If I understand correctly, here
the preserved "structure" is the conservation. In literature, "structure-preserving" means
the ROM solution preserves the structure of the FOM solution.
In this manuscript, the derived SP-LSVT is in conservative form. However, we need to
notice that, even the standard POD-Galerkin ROM can also be written in a conservative
from if we choose the conserved variables as the solution variables. Specific numerical
implementations need to be taken to ensure structure-preserving property of the standard
POD-Glaerkin ROM.
Regrading this issue, the authors should highlight what specific implementations are used
to guarantee the conservation of mass, momentum and energy, and also why that will
work.

\item It will be very intuitive to show "structure-preserving" property of SP-LSVT ROM, if the
authors could plot the errors of the preserved structures of the ROM w.r.t the FOM, such
as the mass, momentum and energy.

\item The authors could plot the pressure oscillation histories at some monitor points on the
chamber to show the develop of the combustion instability. Pressure oscillation histories of
both the ROM and FOM should be plotted and compared to give the readers an intuitive
concept of the accuracy of the ROM.

\item The use of limiter is usually harmful for the convergence of the implicit time stepping.
Could the authors comment on this issue? It will be clear for this point if the authors can
list the average numbers of sub-iterations in the pseudo-time direction with and without
limiters.

\item The author could use Algorithms in the manuscript to more clearly describe the numerical
methods in Section 5, such as the basic procedures of SP-LSVT and the symmetrization-
preserving implicit Runge-Kutta time stepping.

\end{enumerate}

==> figures/Reviewer2.tex <==
\noindent \textbf{Reviewer 2's comments}

\noindent The paper provides a detailed study of reduced-order models (in discrete time) for several combustion applications, which is certainly of interest to the JCP community. The numerical portion is quite extensive and interesting, especially for an application of this caliber. The paper reads fluent. However, my main concern is about properly embedding this work into the existing literature: there are many existing works that are very relevant and related, yet not mentioned.\\


\noindent \textbf{Major comments}
\begin{enumerate}
        \item The introduction could benefit from a more comprehensive review of the literature. Several important works are missing, and in other areas, some of the later literature is cited, but not the papers where the ideas originated. For example:
        \begin{itemize}
                \item A common approach to basis adaptation is Principal Interval Decomposition [Principal interval decomposition framework for POD reduced‐order modeling of convective Boussinesq flows, Borggaard/San] that is very relevant to the discussion of adaptive bases. 
                \item The stabilized Galerkin via eigenvalue reassignment has been addressed much earlier than Rezaian et al, namely by Kalashnikova et al, CMAME, 2014. 
                \item The statement on p.2. ``balanced proper orthogonal decomposition technique [15,16] uses balancing transformations to derive numerically-stable ROMs" is misleading in this reviewers opinion. The two BPOD papers do not show stability of the ROMS--unless I am mistaken. The stability of balanced truncation (not balanced POD) goes back to [ L. Pernebo and L. Silverman, "Model reduction via balanced state space representations," IEEE Trans. Auto. Control, vol. 27, no. 2, pp. 382-387, 1982.]
                \item The introduction mentions variable transformations as a key ingredient, but mentions no related literature. Thus it appears that this is a new idea of the authors. I believe this has been explored elsewhere for decades [such as Hughes/Franca/Mallet 1986, Kerner 1981, McCormick 1976] but also more recently in [Hassler/Ranno/Behr CMAME 2020] and [Kramer/Willcox, AIAA 2019], [Swischuk et al, AIAA 2020] and many others.
        \end{itemize}
        \item In Section~4, the authors show a stability result for linear systems. While this is in discrete time, results for continuous time have been explored, see [Stability Preservation in Projection-based Model Order Reduction of Large Scale Systems by Lohmann and co-authors]. Those results should be discussed and cited. 
        %
        \item The discussion on the use and benefits of variable transformations in Section 5.1. and 5.2. entirely mirrors the discussion in [Kramer \& Willcox 2020], [Swischuk et al., AIAA 2020], [Qian et al., Physica D, 2020] and many others (listed above as well), yet no references are provided. 
        \item In Section 7.1., when using such a large number of modes, do the authors observe a loss of orthogonality in the modes? Which algorithms are used when computing the SVD? Loss of accuracy of orthonormalization has been analyzed, e.g., in [L. Giraud, J. Langou, M. Rozloznik and J. van den Eshof, Rounding error analysis of the classical Gram-Schmidt orthogonalization process, Numer. Math., 101 (2005), 87-100.] 
\end{enumerate}

\noindent \textbf{Minor comments}
\begin{enumerate}
        \item Notation: $\sigma_j$ is at times used for singular value of the snapshot matrix (e.g, eq 71) and other times (Section 7.1.3) as the singular values of the ROM matrix. Maybe sub/superscripts would be good to distinguish. 
\end{enumerate}

==> figures/StandardROM.tex <==
\section{Standard Model Reduction}
\label{StandardROM}
In this section, we introduce the standard Galerkin and least-squares Petrov-Galerkin (LSPG) projection methods for developing ROMs of the governing equations in Eq.~\ref{cfd:discretized}. 

\subsection{Construction of Proper Orthogonal Decomposition Bases} %for Conservative Variables}
\label{pod:consv}
In both approaches, the state $\mathbf{q}$ is expressed in a trial space $\mathcal{V} \triangleq \text{Range}(\mathbf{V})$, where $\mathbf{V} \in \mathbb{R}^{\numDOF \times \numSolModes}$ is the trial basis matrix.   We define   $\mathbf{q}^\prime(\timeVar) \triangleq \mathbf{q}(\timeVar)-\mathbf{q}_\text{ref}$, where $\mathbf{q}_\text{ref}$ is a reference state. Possible reference states include the initial FOM solution, $\mathbf{q}_\text{ref} = \mathbf{q}(\timeVar = \timeVar_0)$, or the time-averaged FOM solution, $\mathbf{q}_\text{ref} = \frac{1}{\Delta \text{T}}\int_{\timeVar_0}^{\timeVar_0 +\Delta \text{T}} \mathbf{q}(\timeVar)\text{dt}$. 

We then seek a representation  $\mathbf{\tilde{q}}: [0,T] \rightarrow \mathcal{V}$ such that
\begin{equation}
   \mathbf{P} ( \mathbf{\tilde{q}}(\timeVar) - \mathbf{q}_\text{ref} ) = \mathbf{V}\mathbf{q}_r(\timeVar),
    \label{pod:expansion_consv}
\end{equation}
where $\mathbf{q}_r: [0,T] \rightarrow \mathbb{R}^{\numSolModes}$ is the reduced state with $\numSolModes$ representing the number of trial basis modes. In this work, $\mathbf{V}$ is computed via the proper orthogonal decomposition (POD)~\cite{Lumley1997} from the singular value decomposition (SVD), which is a solution to
\begin{equation}
  \min_{\mathbf{V} \in \mathbb{R}^{\numDOF \times \numSolModes}} ||\mathbf{Q}-\mathbf{V}\mathbf{V}^T \mathbf{Q} ||_F\ \ s.t. \ \ \mathbf{V}^T \mathbf{V} = \mathbf{I},
    \label{pod:orthogonality_consv}
\end{equation}
Here, $\mathbf{Q}$ is a data matrix in which each column is a snapshot of the solution  $ \mathbf{q}^\prime $ at different time instances. 
A scaling matrix, $\mathbf{P} \in{\mathbb{R}^{\numDOF \times \numDOF}}$, must be applied to  $\mathbf{q}'$ such that the variables corresponding to different physical quantities in the data matrix $\mathbf{Q}$ have similar orders of magnitude. Otherwise, $\mathbf{Q}$ may be biased by physical quantities of higher magnitudes (e.g. total energy). In this work, we normalize all quantities by their $L^2$-norm, as proposed by Lumley and Poje~\cite{Lumley1997}
\begin{equation}
    \mathbf{P} = diag\left(\hat{\mathbf{P}}_1,\ldots,\hat{\mathbf{P}}_i,\ldots,\hat{\mathbf{P}}_{\numCells}\right),
    \label{pod:normalization_consv}
\end{equation} 
where $\hat{\mathbf{P}}_i=diag\left( \varphi^{-1}_{1,norm}, \ldots , \varphi^{-1}_{\numVars,norm} \right)$. Here, $\varphi_{\normVarIdx,norm}$ represents the $\normVarIdx^{th}$ state  variable and
\begin{equation}
    \varphi_{\normVarIdx,norm}={\frac{1}{\Delta \text{T}}\int^{t_0+\Delta \text{T}}_{\timeVar_0}\frac{1}{\Omega}\int_{\Omega}\varphi'^2_\normVarIdx(\mathbf{x}, \timeVar)\text{d}\mathbf{x}\text{dt}}.
\end{equation} 


\subsection{Galerkin Projection}
\label{galerkin_rom}
Model reduction via Galerkin projection is formulated for the continuous-time representation of the FOM (Eq.~\ref{cfd:discretized}). This is done by first scaling Eq.~\ref{cfd:discretized} using the scaling matrix $\mathbf{P}$, then projecting onto the test space $\mathcal{V}$
\begin{equation}
    \mathbf{V}^T \mathbf{P} \frac{\text{d}\mathbf{q}}{\dTimeVar}=\mathbf{V}^T \mathbf{P} \mathbf{f}\left(\mathbf{q}, \timeVar \right).
    %\mathbf{V}^T \mathbf{H}^2 \frac{\text{d}\mathbf{q}_p}{\text{dt}}=\mathbf{V}^T \mathbf{H}^2 \mathbf{\hat{f}}\left(\mathbf{q}_p,t\right).
    \label{rom:galerkin}
\end{equation}
This specification that the trial and test spaces are identical defines Galerkin projection. The scaling of Eq.~\ref{cfd:discretized} is necessary to ensure that each equation makes similar contributions to the reduced system after projection. Otherwise, the reduced system may be biased by equations for quantities of higher magnitudes (e.g. the energy equation), exacerbating floating-point errors. With the low-rank representation in Eq.~\ref{pod:expansion_consv}, $\mathbf{\tilde{q}}(\timeVar) \triangleq \mathbf{q}_\text{ref}+\mathbf{P}^{-1}\mathbf{V}\mathbf{q}_r(\timeVar)$, substituted into Eq.~\ref{rom:galerkin}, a reduced-order ODE system can be obtained 
\begin{equation}
    \frac{\text{d}{\mathbf{q}_r}}{\dTimeVar} = \mathbf{V}^T \mathbf{P} \mathbf{f}\left( \mathbf{\tilde{q}, \timeVar} \right), \ \ \mathbf{q}_r(0) = \mathbf{V}^T\mathbf{q}_0.
    \label{rom:galerkin_ode}
\end{equation}
 The dimension of the ROM ODE is $\numSolModes$, which can be orders of magnitudes smaller than  $\numDOF$  in Eq.~\ref{cfd:discretized}.

\subsection{Least-squares Petrov-Galerkin Projection}
\label{slspg_rom}
Least-squares Petrov-Galerkin (LSPG) projection~\cite{Carlberg2017} is formulated from the discrete-time representation of Eq.~\ref{cfd:discretized}. The objective of LSPG is to minimize the fully-discrete FOM equation residual, $\mathbf{r}$, defined in Eqs.~\ref{EqRes:LinearMultiStep} and~\ref{EqRes:RK}, with respect to the state, $\mathbf{q}$, as approximated in the trial space $\mathcal{V}$,  $\mathbf{\tilde{q}} = \mathbf{q}_\text{ref}+\mathbf{P}^{-1}\mathbf{V}\mathbf{q}_r$. %It should be noted that $\mathbf{r}(\mathbf{q}^n) = 0$ but $\mathbf{r}(\mathbf{\tilde{q}}^n)$ does not necessarily equal to zero. Therefore, 
The problem statement of LSPG is to seek a solution to the minimization problem
\begin{equation}
    \tilde{\mathbf{q}}^\iterIdx \triangleq  \arg \min_{ \tilde{\mathbf{q}}^\iterIdx \in \textrm{Range}(\mathbf{V})} \norm{\mathbf{P}\mathbf{r}(\mathbf{\tilde{q}}^\iterIdx)}^2,
    \label{rom:slspg_def}
\end{equation}
with the equation residual, $\mathbf{r}$, scaled by $\mathbf{P}$ such that each equation in $\mathbf{r}$ has similar contributions to the minimization. The norm used is the the Euclidean vector-induced matrix norm $L_{2,2}$, which we will represent by $\norm{\cdot}.$

The solution of this minimization problem seeks to satisfy
\begin{equation}
    (\mathbf{W}^\iterIdx)^T \mathbf{P} \mathbf{r}(\mathbf{\tilde{q}}^\iterIdx) = 0,
    \label{rom:slspg_proj}
\end{equation}
where $\mathbf{W}^{\iterIdx}$ is the Petrov-Galerkin projection test basis given by
\begin{equation}
    \mathbf{W}^\iterIdx = \frac{\partial\mathbf{P}\mathbf{r}(\mathbf{\tilde{q}}^\iterIdx)}{\partial\mathbf{q}^n_r}.
    \label{rom:slspg_w}
\end{equation}

%We now develop LSPG ROMs for the linear multi-step and Runge--Kutta time integrators introduced in Section~\ref{fom}. 
For linear multi-step methods, the equation residual in Eq.~\ref{EqRes:LinearMultiStep} yields the test basis
\begin{equation}
    \mathbf{W}^\iterIdx = \mathbf{P} \left( \mathbf{I} - \dt \beta_0 \tilde{\mathbf{J}}^\iterIdx \right) \mathbf{P}^{-1} \mathbf{V},
    \label{rom:slspg_w_LinearMultistep}
\end{equation}
where $\tilde{\mathbf{J}}^\iterIdx = \left[\partial\mathbf{ f }/\partial\mathbf{q}\right]^\iterIdx_{\mathbf{q}=\tilde{\mathbf{q}}}$.  For explicit schemes ($\beta_0 = 0$), $\mathbf{W}^\iterIdx = \mathbf{V}$, thus reverting to Galerkin projection. Similarly, for Runge--Kutta methods, the equation residual in Eq.~\ref{EqRes:RK} yields the test basis
\begin{equation}
    \mathbf{ W }^\iterIdx = \mathbf{V},
    \label{rom:slspg_w_RK}
\end{equation}
which is identical to the trial basis as in Galerkin projection. %It should be pointed out that the test basis $\mathbf{W}$ is the same for both explicit and implicit Runge--Kutta methods.

==> figures/commands.tex <==
\newcommand{\error}{\mathbf{e}}
\newcommand{\RHSbasisvec}{\mathbf{U}}
\newcommand{\sampvec}{\mathbf{P}}
%\newcommand{\norm}[1]{\big| \big| #1 \big| \big|_2 }
\newcommand\norm[1]{\left\lVert#1\right\rVert_2}

\newcommand{\PDEspace}{\mathbb{R}^N \times [0,T]}
\newcommand{\xjic}{x_{0j}}
\newcommand{\icspace}{\mathbb{R}^N}
\newcommand{\icspacecoarse}{\tilde{\MC{H}}}
\newcommand{\icspacefine}{\MC{H}'}

\newcommand{\errorcoarse}{\mathbf{\tilde{e}}}
\newcommand{\errorfine}{\mathbf{e'}}

\newcommand{\velocity}{\mathbf{f}}

\newcommand{\mat}[1]{{\bf #1}}
\newcommand{\mb}[1]{{\mathbf{#1}}}

\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\BG}{\boldsymbol}
\newcommand{\be}{\ensuremath{{\boldsymbol\beta}}\xspace}
\newcommand{\ret}{\ensuremath{ Re_{\theta} \xspace}}
 \newcommand{\eqnref}[1]{(\ref{#1})}
 \newcommand{\class}[1]{\texttt{#1}}
 \newcommand{\package}[1]{\texttt{#1}}
 \newcommand{\file}[1]{\texttt{#1}}
 \newcommand{\BibTeX}{\textsc{Bib}\TeX}
%\long\def\comment#1\endcomment{}
\newcommand{\alf}{\ensuremath{{\boldsymbol\alpha}}\xspace}

\newcommand{\errorcoarsegen}{\mathbf{\tilde{a}^e}}
\newcommand{\errorfinegen}{\mathbf{\tilde{a}^e}}
\newcommand{\MC}{\mathcal}

%\newcommand{\mbx}{{\mb{x}}}
%\newcommand{\mby}{{\mb{y}}}

\newcommand{\mbx}{{\mb{q}}}
\newcommand{\mby}{{\mb{s}}}
\newcommand{\mbxr}{{\mb{q}_r}}
\newcommand{\mbyr}{{\mb{s}_r}}


\newcommand{\mbr}{{\mb{Q}}}
\newcommand{\mbs}{{\mb{S}}}
\newcommand{\mbj}{{\mb{J}}}
\newcommand{\mbi}{{\mb{I}}}
\newcommand{\mbv}{{\mb{V}}}
\newcommand{\mbu}{{\mb{U}}}
\newcommand{\mbp}{{\mb{P}}}
\newcommand{\mbb}{{\mb{B}}}

\newcommand{\mbw}{{\mb{W}}}
\newcommand{\rx}{{\mb{r}_\mbx}}
\newcommand{\ry}{{\mb{r}_\mby}}

\newcommand{\mbg}{{\boldsymbol{\Gamma}}}
\newcommand{\mf}{{\mb{f}}}


\newcommand{\Hfine}{{\MC{H}^{\prime}}}
\newcommand{\Hcoarse}{\tilde{\MC{H}}}
\newcommand{\trieq}{\overset{\Delta}{=}}
\newcommand{\wfullvec}{{\mathbf{w}}}
\newcommand{\ufullvec}{{\mathbf{u}}}
\newcommand{\ufinevec}{{\mathbf{u}^{\prime}}}
\newcommand{\ucoarsevec}{\tilde{\mathbf{u}}}
\newcommand{\vfinevec}{{\mathbf{V}^{\prime}}}
\newcommand{\vcoarsevec}{\tilde{\mathbf{V}}}
\newcommand{\vmidvec}{\hat{\mathbf{V}}}
\newcommand{\vfullvec}{{\mathbf{V}}}

\newcommand{\Psifinevec}{{\mathbf{\psi}^{\prime}}}
\newcommand{\Psicoarsevec}{\tilde{\mathbf{\psi}}}
\newcommand{\Psifullvec}{{\mathbf{\psi}}}

\newcommand{\itermaxLinMS}{\ensuremath{l}}      % max number of linear multistep steps
\newcommand{\itermaxRK}{\ensuremath{s}}         % max number of RK steps
\newcommand{\iterIdx}{\ensuremath{n}}           % physical iteration index
\newcommand{\subIdx}{\ensuremath{k}}            % subiteration index
\newcommand{\normVarIdx}{\ensuremath{v}}        % scaling matrix variable index
\newcommand{\varIdx}{\ensuremath{i}}            % generic state variable indexing 
\newcommand{\numDOF}{\ensuremath{N}}            % total number of degrees of freedom
\newcommand{\numCells}{\ensuremath{N_{vol}}}    % number of finite volume cells
\newcommand{\numVars}{\ensuremath{N_{var}}}     % number of state variables
\newcommand{\numSolModes}{\ensuremath{n_p}}     % number of modes retained in solution trial basis
\newcommand{\numResModes}{\ensuremath{n_d}}     % number of modes in residual basis
\newcommand{\numSamps}{\ensuremath{n_s}}
\newcommand{\timeVar}{\text{t}}                 % time variable
\newcommand{\dt}{\ensuremath{\Delta \text{t}}}  % physical time step size
\newcommand{\dTimeVar}{\text{dt}}               % change in time variable in ODE
\newcommand{\dPTimeVar}{\ensuremath{\text{d}\tau}} % change in pseudo-time variable in ODE
\newcommand{\dtau}{\ensuremath{\Delta \tau}}    % pseudo-time step size

\newcommand{\water}{\ensuremath{\text{H}_2\text{O}}}
\newcommand{\oxygen}{\ensuremath{\text{O}_2}}
\newcommand{\methane}{\ensuremath{\text{CH}_4}}
\newcommand{\carbonDiox}{\ensuremath{\text{CO}_2}}

\newcommand{\crw}[1]{{\color{ForestGreen}#1}}

==> figures/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
A comprehensive projection-based reduced-order model (ROM) formulation is presented for multi-scale and multi-physics problems. A structure-preserving least-squares formulation with variable transformation (SP-LSVT) is derived to provide global stability enhancement. The new formulation builds on recent developments in least-squares-based ROMs~\cite{Carlberg2017,GrimbergPROM2020}, and relies on least-squares minimization of the discrete equation residuals to guarantee symmetrization and discrete consistency with the full-order model at both the physical-time and the sub-iteration levels. It allows for the selection of arbitrary (but complete) solution variables while preserving the governing equations in conservative form so that the consistency between FOM and ROM is achieved at the fully discrete level. It is applicable to both implicit and explicit time integrators (in contrast to LSPG projection~\cite{Carlberg2017,GrimbergPROM2020}, which requires implicit time integrators) and provides more flexibility in constructing and computing the ROMs. Detailed evaluations of the SP-LSVT formulation are performed based on a representative 2D reacting flow problem with a stiff chemical kinetic model that can often result in challenging numerical robustness issues even for full-order models. The SP-LSVT formulation is shown to produce ROMs with significantly improved stability and accuracy over the standard projection-based ROM techniques. The SP-LSVT ROMs remain stable and exhibit largely monotonic error decay with respect to the number of modes included in the trial basis. To address a gap in the literature, we present a proof of linear stability of least-squares-based ROMs for linear time invariant systems. This is followed by a numerical analysis of linearized version of the reacting flow equations, further confirming the linear stability and improved conditioning offered by the SP-LSVT procedure.

%More importantly, the major features of the proposed formulation are:
%\begin{enumerate}
%  \item It allows arbitrary selection of solution variables while preserving the governing equations in conservative form so that the consistency between FOM and ROM can be achieved on fully discrete level.
%  \item It is applicable to both implicit and explicit time integrators and provides more flexibility in constructing and calculating the ROMs.
%  \item Evaluations on representative 2D reacting flow problems demonstrate significant enhancement in global stability compared to standard Galerkin and LSPG methods.
  %\item For both 2D and 3D reacting flow test problems, it shows less sensitivity to ROM computing time steps. It is demonstrated that the SP-LSVT ROMs are able to provide similar accuracy even with 10 times of the full order model time steps, which provides further computational efficiency.
%\end{enumerate}

For local stabilization, physical realizability in reacting flow ROMs is improved by enforcing limiters on the temperature and species mass fraction fields to mitigate the production of local spurious oscillations near sharp gradients. %In previous work by the current authors~\cite{HuangAIAAJ2019}, the temperature limiter was demonstrated to be necessary for maintaining stable and accurate reacting flow ROMs, and also proved important for ROMs of hypersonic applications~\cite{BloniganHypersonics} with strong temperature gradients present. 
The importance of a species mass fraction limiter is demonstrated for both 1D and 2D reacting flow problems with stiff chemical kinetics. It is shown to be especially effective in improving the accuracy of heat release rate and flame  speed predictions,  both of which are important quantities of interest in reacting flows. 

%\st{for problems with stiff chemical kinetics}.


Enhancement of computational efficiency is demonstrated in a 3D reacting single injector problem via hyper-reduction using gappy POD.  A factor of 319 speedup in wall clock time and 638 in CPU time can be achieved with SP-LSVT ROM on a 1\% sampled mesh, calculated using an explicit time integrator and a physical time step 10 times that of the FOM.

Finally, the capability of the SP-LSVT ROM in predicting the  dynamics beyond the training window is assessed in the 3D case. Though both the SP-LSVT ROMs  are able to provide reasonably accurate predictions of the pressure field,  future-state predictions of the temperature field remain challenging. This is, however, not a limitation of the SP-LSVT procedure, as the projection error is itself high at the future state -- a consequence of a static linear basis approximation. To improve on this, adaptive bases~\cite{peherstorfer2015online,PeherstorferADEIM} or non-linear manifold ROMs~\cite{LeeNonlinearManifold2020} can be leveraged with the SP-LSVT formulation. Future work will also include explorations of explicit constraint preservation (e.g. enforcing conservation~\cite{CarlbergConsvLSPG}).

%{\color{red} Talk about another direction for future work: explicit constraint preservation like what Carlberg did using aggregated volumes for conservation}

==> figures/formulation.tex <==
\input{FullOrderModel.tex}
\input{StandardROM.tex}
\input{Proofs.tex}
\input{LSPG-VT.tex}
\input{HyperReduction.tex}
\input{Limiters.tex}







==> figures/intro.tex <==
\section{Introduction}
\label{intro}
With  advances in computing architectures and computational algorithms, high-fidelity multi-physics simulations are becoming integral to the analysis and design of complex systems. A pertinent example is that of reacting flow simulations~\cite{adityaDNS, OefeleinSupercritical} which play an important role in the investigation and understanding of combustion dynamics in propulsion systems operating at high pressures and temperatures, providing details  which cannot be quantitatively accessed through experiments. Accurate and efficient modeling of combustion dynamics in a practical environment has the potential to improve engine performance and reduce failures. %Though modern computational capability has moved beyond the empirically-based design analyses of the past, high-fidelity simulations of full-scale practical combustors remain out of reach for day-to-day engineering design applications. 
 Large eddy simulations (LES) of combustion dynamics -- even for small-scale engines  ~\cite{UrbanoLES2016} -- typically require $O(10^7)$ CPU-hours per simulation, and are thus impractical in many-query applications such as engineering design and uncertainty quantification. %Therefore, for simulation-based design to be a reality, accurate and efficient modeling methodologies are imperative. 
In the present work, we develop model reduction techniques to achieve efficient and accurate simulations of complex multi-physics problems, and use rocket combustion examples to motivate and evaluate our algorithms.

Projection-based reduced-order models~\cite{Lumley1997,Graham1997,Lucia2003} have proven to be effective in reducing partial differential equations (PDE)-based dynamical systems to low-dimensional manifolds and have been successfully applied in problems such as flow control~\cite{Barbagallo2012,Barbagallo2009,Barbagallo2011} and aeroelasticity~\cite{Lieu2007,Lucia2004}. 
%More recent studies have extended ROMs to reacting flow problems~\cite{MunipalliRBM,Huang2007} and preliminary explorations of the POD/Galerkin technique have been carried out~\cite{Huang2014,Huang2015} using a simple 1D solver to establish a basic approach for ROM construction and its characteristics in reacting flows.
%
%This work is part of a larger initiative in which the authors are developing a Multi-Fidelity Framework using Reduced Order Modeling (ROM) to enable efficient modeling of combustion dynamics in practical full-scale engines. Using a rocket engine as an example, it should be noted that complex flow phenomena are limited to the region in and around the injector element, where the propellants mix and react through actions of shear, swirl, and/or direct impingement. In large, high-performance rocket engine combustors, where the problem of instability is particularly severe, hundreds of injector elements are typically used. The design and operation of these individual elements control the spatio-temporal aspects of mixing, reaction, and the overall heat addition field. Although the number of injector elements is large (which precludes application of high-fidelity methods to the entire combustor), the elements themselves are rather small (the largest are on the order of 1 cm). This fact can be used to an advantage by restricting the detailed characterization of the unsteady flowfield and its response to flow perturbations to one or a small set of injector elements. Then, a generalized reduced order model (ROM) for  injector elements can be extracted from the simulations and implemented in multi-fidelity design framework suitable for engineering analysis. The idea of such a multi-Fidelity framework has been successfully demonstrated in simpler model problems~\cite{Huang2019,Xu2019}.
When applied to complex multi-scale problems that involve transport phenomena such as convection, it is well-recognized that projection-based ROMs suffer from accuracy and stability issues. These issues may arise from the inherent lack of numerical stability in projection method itself (e.g. Galerkin projection~\cite{Rempfer2000}), mode truncation (e.g. removal of low-energy spatial modes~\cite{Bergmann2009}), or simplifications of model equations~\cite{Noack2005}. Several remedies have been proposed in the literature. In linear systems, the balanced proper orthogonal decomposition technique~\cite{Rowley2005,Willcox2002} uses balancing transformations to derive numerically-stable ROMs. 

The use of adaptive bases~\cite{peherstorfer2015online,PeherstorferADEIM,CarlbergAdaptiveBasis2015,EtterAdaptiveBasis2020} and projection onto non-linear manifolds via deep convolutional autoencoders~\cite{LeeNonlinearManifold2020} have also been investigated to mitigate ROM accuracy and stability issues. Another group of studies address stability issues from the perspective of closure modeling, accounting for the effect of truncated ROM dynamics based on the resolved ROM dynamics (analogous to the closure problem in LES). Bergmann et al.~\cite{Bergmann2009} proposed to use residuals of the full-order models to account for the absence of low-energy dissipative spatial modes. Lucia et al.~\cite{Lucia2003} demonstrated the effectiveness of constructing stable ROMs by including additional artificial dissipation terms. Rezaian et al.~\cite{rezaian2020hybrid} used implicit sub-space correction and eigenvalue reassignment to stabilize Galerkin ROMs of compressible flows with shocks and vortex shedding phenomena.


Variational multi-scale (VMS) closure models~\cite{SanVMS2015,IliescuVMS2014,StabileVMS2019} for projection-based ROMs have been demonstrated to offer stabilization for multi-scale problems. Parish et al.~\cite{parish2017non,parish2017dynamic} leveraged the Mori–Zwanzig (MZ) formalism to develop a closed representation of the unresolved scales. Extended to projection-based ROMs~\cite{Parish2019}, the method is referred to as the Adjoint Petrov–Galerkin (APG) method. The Markovian first order approximation to the memory kernel yields a technique that is analogous to adjoint-stabilization~\cite{hughes1995multiscale} in the finite element community.

Researchers have also attempted to leverage the underlying numerical discretization to improve ROM stability. Rowley et al.~\cite{Rowley2004} pointed out that defining a physically-meaningful inner product to obtain low-dimensional manifolds (e.g. proper orthogonal decomposition bases) can yield  a quadratic reduced system that is more stable and much simpler to implement for model reduction of compressible flows. Barone et al.~\cite{Barone2008,Barone2009JCP} proposed to stabilize the reduced system by symmetrizing the higher-order PDE with a preconditioning matrix, and also highlighted the importance of formulating a proper inner product in preserving stability in the reduced system. For aeroelastic applications, Amsallem and Farhat~\cite{Amsallem2014} have shown the advantages of using the descriptor form over the non-descriptor form of the governing equations. While these methods can enable stable ROMs, they can compromise the conservative properties of the governing equations during the model reduction procedure. Afkham et al.~\cite{Afkham2020} highlighted the importance of preserving the conservative form of the governing equations in ROM development. 

Following developments in the finite element community (e.g. the Galerkin Least-Squares technique of stabilization~\cite{LSFEM}), Carlberg et al.~\cite{carlberg2013gnat,Carlberg2017}  demonstrated that minimizing the least-squares residual of the projected solution yields stabilized non-linear ROMs. This technique is referred to as least-squares Petrov-Galerkin (LSPG) projection. The GNAT method~\cite{carlberg2013gnat} extends hyper-reduction to LSPG projection.  Strategies have also been developed to explicitly enforce desirable properties such as discrete conservation~\cite{CarlbergConsvLSPG}. Grimberg et al.~\cite{GrimbergPROM2020} demonstrated improved stability, accuracy and efficiency of hyper-reduced LSPG ROMs (HPROMs) in the context of convection-dominated turbulent flows.  In practice, least-squares-based techniques have been restricted to implicit time integration schemes, as applying residual minimization to an explicit time integrator results in a test basis that is  identical to the trial basis. 


%{\color{red} What Charbel calls as HPROMs is also LSPG.. mention that and don't attribute it to just Carlberg}.

%{\color{red} Need more references. Check Eric's APG paper for more content. Of course, don't repeat the same statements, but use some of the papers to draw conclusions \color{blue}{I highlighted a bit more on the importance of preserving the conservative form of the governing equations and the fact that the standard LSPG will lose it when choosing non-conservative solution variables.}}

The above investigations have been demonstrated to be effective in the applications pursued in the respective publications. Many multi-scale, multi-physics contexts, such as reacting flows, further exacerbate accuracy and robustness issues  with high numerical stiffness arising from the chemical kinetics. This stiffness can lead to  Jacobian matrices with high condition numbers $O(10^{12})$, and may produce many issues even in full-order models~\cite{StoneKinetics}. For instance, a recent investigation~\cite{HuangAIAAJ2019} has identified the appearance of localized spurious oscillations near sharp, dispersed flame fronts as a major contributor to the stability issues in reacting flow ROMs. These oscillations are a consequence of under-resolution, or the inability of the ROM to resolve resolve sharp flame fronts, and can often lead to features such as negative temperatures (i.e. T $\leq$ 0 K) that terminate the calculations. A temperature limiter was required to improve ROM robustness even in relatively simple reacting flow configurations. Similar ideas of enforcing physical realizability were also employed by Blonigan et al.~\cite{BloniganHypersonics} for hypersonic flow applications in which strong temperature gradients are present.

In the present work, we develop a comprehensive framework for projection-based reduced-order model development for complex multi-scale applications to achieve improved robustness and computational efficiency. Particularly, we introduce a structure-preserving variable transformation and leverage least-squares minimization~\cite{Carlberg2017} to achieve global stabilization. To promote local stability, we enforce physical realizability on both temperature and species mass fraction fields. This method achieves discrete consistency and symmetrization at the sub-iteration level, {\color{blue} results in well-conditioned ROMs}, and allows for the use of implicit and explicit time integrators. We refer to our new formulation as the structure-preserving least-squares with variable transformation (SP-LSVT) technique. Detailed evaluations of the SP-LSVT technique and comparisons with Galerkin and LSPG projection are presented in challenging reacting flow applications.
 
     %\item The introduction of physical realizability enforcement via imposing limiters on temperature and species mass fractions for local stability and accuracy enhancement. It is demonstrated in the current work that even with the global stabilization method (SP-LSPG), the local physical realizability is not guaranteed and needs to be enforced via limiters. 
  %The numerical tests demonstrate that the proposed SP-LSVT formulation is more accurate and robust compared to the Galerkin and the standard LSPG formulations. A decrease in computational cost by two orders of magnitude in computational efficiency is achieved with reasonable future state prediction capabilities in a 3D reacting flow problem at high pressure and high temperature conditions.


The remainder of the paper is organized as follows. Section~\ref{fom} presents  the full-order model (FOM) and time discretization. Section~\ref{StandardROM} reviews the procedure for standard model reduction via Galerkin and LSPG projection. Identifying a gap in the literature, Section~\ref{proof} presents a proof of linear stability of least-squares-based ROMs. Section~\ref{SPLSPG} introduces the selection of transformed solution variables, and the procedure for SP-LSVT projection to achieve symmetrization and discrete consistency. Section~\ref{limiters} discusses a limiter-based strategy to improve local robustness. Section~\ref{results} presents numerical results  and analysis for ROMs of benchmark reacting flow problems and assesses their accuracy, robustness, and efficiency. In Section~\ref{sec:conclusion}, we provide concluding remarks and perspectives.


==> figures/results.tex <==
\section{Numerical Results and Analysis}
\label{results}
\input{results_2DSingleInjector.tex}
\input{results_3DSingleInjector.tex}


==> figures/results_2DSingleInjector.tex <==

To assess the capabilities of projection-based ROMs in predicting complex multi-scale multi-physics problems, such as reacting flows, two rocket combustor configurations are established based on a generic laboratory-scale single injector combustor~\cite{YuJPP}. The first configuration is a simplified two-dimensional representation of the injector. This case is used to assess the accuracy and robustness of different ROM formulations, including Galerkin projection, LSPG projection, and the SP-LSVT formulation. The second configuration is a full three-dimensional representation of the injector used in physical experiments, and is used to evaluate the computational efficiency and predictive capabilities of the SP-LSVT ROM formulation. It should be pointed out that numerical results for the SP-LSVT ROM reported here were obtained using the physical time formulation (Section~\ref{lspg-vt}). The dual-time formulation (Section~\ref{lspg-vt-dualtime}) was also found to produce very similar results, and are not reported here for brevity.

The computational infrastructure used for the full- and reduced-order models solves conservation equations for mass, momentum, energy and species  transport in a fully coupled way using the  in-house CFD code, the General Mesh and Equation Solver (GEMS). GEMS  has been used to model a variety of complex, practical reacting flow problems~\cite{HarvazinskiPoF,HuangLDI}. More details of the FOM equations can be found in~\ref{appendix:fom_eq}. The FOM employs a cell-centered second-order accurate finite volume method for spatial discretization. The Roe scheme~\cite{Roe1981} is used to evaluate the inviscid fluxes and a Green-Gauss gradient reconstruction procedure~\cite{MitchellReconScheme} is used to compute the face gradients and viscous fluxes. A gradient limiter by Barth and Jespersen~\cite{barth1989} is used to preserve monotonicity for flow fields with strong gradients. A ghost cell formulation is used for treatment of boundary conditions. Time integration for all FOM simulations uses the implicit second-order accurate backwards differentiation formula with dual time-stepping.

It should be recognized that in the case of reacting flow modeling, the chemical source terms in the species transport equations often lead to extreme numerical stiffness due to the kinetic model~\cite{WestbrookDryer}. The example in~\ref{appendix:species_oscillations} illustrates this problem. This stiffness is the result of rapid production or destruction of species at the microseconds timescale, which requires a very small time step for accurate resolution. More importantly, it can also produce stiff Jacobians with a high condition number, which can be as high as $O(10^{12})$ for high-pressure and high-temperature conditions. Solving the resulting linear system is very challenging, even at the FOM level.

\subsection{2D Reacting Injector}
\label{2d:injector}
 We begin with a 2D-planar representation of the generic laboratory-scale rocket combustor~\cite{YuJPP}. This simplified model allows ROM capabilities to be evaluated in great detail without incurring exorbitant computational cost, while maintaining the essential physics of interest. The configuration is shown in Fig.~\ref{2d:geometry} and consists of a shear coaxial injector with an outer passage, $T_1$, that introduces fuel near the downstream end of the coaxial inner passage, $T_2$, that feeds oxidizer to the combustion chamber. The $T_1$ stream contains gaseous methane (100\% \methane) at 300 K. The $T_2$ stream is 42\% gaseous \oxygen\ by mass and 58\% gaseous \water\ by mass at 700 K. 

Operating conditions in the combustion chamber are maintained similar to conditions in the laboratory combustor~\cite{YuJPP,YuPhD}, with an adiabatic flame temperature of approximately 2,700 K and a mean chamber pressure of 1.1 MPa. Both the $T_1$ and $T_2$ streams are fed with constant mass flow rates, 0.37 kg/s and 5.0 kg/s, respectively. A non-reflective boundary condition is imposed at the downstream end to allow acoustic waves to properly exit the domain and control acoustic effects on the combustion dynamics. A sinusoidal pressure perturbation at 2,000 Hz, with amplitude 10\% of the mean pressure, is imposed at the downstream boundary. Transport of four chemical species (\methane, \oxygen,  \water, \carbonDiox) is modeled. The chemical reaction is modeled by the global single-step methane-oxygen reaction recommended by Westbrook and Dryer~\cite{WestbrookDryer}:
$
   \methane + 2 \oxygen \rightarrow \carbonDiox + 2 \water.
$
The chemical species are treated as thermally perfect gases.

As reported by the current authors~\cite{Huang2018Jan}, stable and accurate reconstruction of FOM solutions with stiff chemistry via projection-based ROMs is highly challenging. To mitigate these difficulties, studies have been performed by the current authors to evaluate ROM performance based on simulations using a reduced Arrhenius pre-exponential factor~\cite{HuangAIAAJ2019} ten times smaller than the value recommended by Westbrook and Dryer~\cite{WestbrookDryer}, producing a discrete system which is far less stiff and more amenable for ROM development and testing. The same dataset has also been used to investigate the use of operator inference learning in constructing ROMs for reacting flow simulations~\cite{Swischuk2020AIAAJ_LL}. It has been reported by the current authors~\cite{HuangAIAAJ2019} that even with this reduced reaction rate, construction of robust and accurate ROMs remains highly challenging and provides a clear example of the additional difficulties engendered when reactions are present. However, the 2D configuration (Fig.~\ref{2d:geometry}) in the current work is simulated with the stiff chemical kinetic model with the original pre-exponential factor to fully assess the capabilities of the proposed ROM framework. Therefore, more challenges are anticipated with the stiff chemical model in the current study.

\begin{figure}
	\centering
	\includegraphics[width=1.0\textwidth]{./figures/2d_geometry.png}
	\caption{Computational configuration of 2D planar reacting  injector simulation.}\label{2d:geometry} 
\end{figure}

Two representative instantaneous snapshots of the 2D reacting single injector FOM solutions are shown in Fig.~\ref{2d:fom_snapshots} to demonstrate the overall characteristics of the flow field and highlight the dominant physics in the problem. The pressure exhibits global dynamics over the entire domain, while the combustion dynamics are characterized by local features like disperse pockets of intense heat release that are intermittently distributed in both space and time. The temperature and heat release rate contours span a wide range of scales, from the small eddies in the shear layers to the large-scale recirculation zone immediately downstream of the the dump plane at $x = 0$ m. More importantly, strong interactions can be identified between pressure and combustion dynamics. When the pressure  is low near the dump plane, high temperature pockets are distributed downstream of the combustor. Alternately, when the pressure is high at the dump plane, high temperature pockets are concentrated closer to the dump plane. These unique features and interactions introduce varying levels of difficulty in constructing a robust ROM.

\begin{figure}
	\centering
	\includegraphics[width=1.0\textwidth]{./figures/2d_fom_snapshots.png}
	\caption{Representative instantaneous snapshots of pressure (top), temperature (middle) and heat release rate (bottom) from FOM simulation of the 2D reacting  injector.}\label{2d:fom_snapshots} 
\end{figure}

The 2D FOM is computed using the second-order accurate  backwards difference formula and dual time-stepping, with a constant physical time step of 0.1 $\mu$s. The entire mesh contains a total of 38,523 finite volume cells with 7 solution variables ($p$, $u$, $v$, $T$, $Y_\text{CH4}$, $Y_\text{O2}$ and , $Y_\text{H2O}$), resulting in a total of 269,661 degrees of freedom. $Y_\text{CO2}$ is computed from the simple relation $\sum_i Y_i = 1$. Snapshots are stored at every physical time step over a duration of 1.0 ms, corresponding to a total of 10,000 snapshots, all of which are used to generate POD modes for ROM construction.

\subsubsection{POD Characteristics}
\label{2d:results-pod_res_energy}

The POD characteristics of the reacting flow problem are first investigated to understand how well the POD trial basis represents the FOM dataset. The representation is evaluated using the POD residual energy: 
\begin{equation}
    \text{POD Residual Energy}(n_p){\%}{=}\left(1-\frac{\sum^{n_p}_{j=1}\sigma^2_j}{\sum^{n_{p,total}}_{j=1}\sigma^2_j}\right)\times{100\%},
    \label{pod:res_energy}
\end{equation}
where $\numSolModes$ is the number of vectors retained in the POD trial basis, and $n_{p,total}$\ (= 10,000) is the total number of snapshots in the dataset. The residual energy as a function of $\numSolModes$, as shown in Fig.~\ref{2d:pod_res_energy}, reveals the information excluded by the POD representation for a given  number of modes. The results show that the first 15 modes must be included to capture approximately 90\% of the total energy, 52 modes recover approximately 99\%, and at least 130 modes are needed to retrieve 99.9\% of the total energy. This slow energy decay is indicative of the significant complexity of the system dynamics. Many fundamental projection-based ROM methodologies are tested on relatively simple problems requiring only $\sim 10$ trial basis modes to achieve 99.9\% POD energy~\cite{LeeNonlinearManifold2020, Barone2009JCP, sanANNClosure}. ROMs for more practical engineering systems, however, generally require $\sim 100$ trial basis modes~\cite{StabileVMS2019, Carlberg2017, GrimbergPROM2020}.
\begin{figure}
	\centering
	\includegraphics[width=0.6\textwidth]{./figures/2d_pod_res_energy.png}
	\caption{POD residual energy distribution for the 2D reacting  injector simulation.}\label{2d:pod_res_energy} 
\end{figure}

\subsubsection{ROM Performance: Galerkin vs. LSPG vs. SP-LSVT}
\label{2d:results-ROM}
The ability of a ROM to accurately model the evolution of the unsteady flow field is measured here in terms of the normalized, time-averaged, and variable-averaged $L^2$ error over the POD trial basis training window

\begin{equation}
    \epsilon = \frac{1}{N_{var}}\sum^{N_{var}}_{\varIdx=1} \frac{1}{n_t}\sum^{n_t}_{\iterIdx=1}\frac{\left\|\mathbf{\tilde{q}}^\iterIdx_{p,\varIdx}-{\mathbf{q}^\iterIdx_{p,\varIdx}}\right\|_2}{\left\|{\mathbf{q}^\iterIdx_{p,\varIdx}}\right\|_2},
    %\text{Global ROM Reconstruction Error}(n_p)=\frac{1}{n_t}\sum^{n_t}_{n=1}\frac{\left\|\mathbf{V}\mathbf{q}^n_r-\mathbf{V}\mathbf{V}^T{\mathbf{Q}'^n_p}\right\|_2}{\left\|{\mathbf{Q}_{p,ref}+\mathbf{V}\mathbf{V}^T{\mathbf{Q}'^n_p}}\right\|_2}
    \label{rom:reconstr_err}
\end{equation}
where $\mathbf{\tilde{q}}^\iterIdx_{p,\varIdx}$ represents the $i^{th}$ solution variable of the state vector, $\mathbf{\tilde{q}}^\iterIdx_{p}$,  at time step $n$ from ROM simulations following Eq.~\ref{pod:expansion_qp}, and $\mathbf{q}^\iterIdx_{p,\varIdx}$ is obtained from FOM solutions. The entire error measure, $\epsilon$, is referred to as the reconstruction error, referring to the accuracy at which the ROM reconstructs the training data..

Figure~\ref{2d:rom_recon_err} presents the ROM reconstruction error  using Galerkin projection, LSPG projection, and the SP-LSVT formulation with different time integration schemes and a varying number of modes retained in the trial basis. Results are shown for total mode numbers ranging from 4 to 100. To obtain a comprehensive assessment of different ROM methods, Galerkin and LSPG ROMs are developed based on both the conservative governing equations (Eq.~\ref{cfd:discretized}) and the non-conservative equations (Eq.~\ref{cfd:discretized_qp_ge}).  ROMs using the former class of method are denoted as ``Galerkin-C'' and ``LSPG-C'', and those using the latter are denoted as as ``Galerkin-N'' and ``LSPG-N''. It is emphasized that Galerkin and LSPG projection are derived based on the premise that the governing equations and the solution variables are consistent  (i.e. the conservative variables $\mathbf{q}$ are chosen as the solution variables for Eq.~\ref{cfd:discretized} and the non-conservative variable $\mathbf{q}_p$ for Eq.~\ref{cfd:discretized_qp_ge}).  On the other hand, SP-LSVT ROMs are developed based on the conservative governing equations with transformed solution variables (Eq.~\ref{cfd:discretized_qp}). 

\begin{figure}
	\centering
	\includegraphics[width=0.6\textwidth]{./figures/2d_rom_recon_error.png}
	\caption{Global ROM reconstruction error comparisons between Galerkin, LSPG and SP-LSVT ROM methods with different time integration schemes for the 2D reacting  injector simulation.}\label{2d:rom_recon_err} 
\end{figure}

All the ROMs in Fig.~\ref{2d:rom_recon_err} are calculated with the temperature limiter introduced in Section~\ref{limiters}, with $T_{min} = 270$ K and $T_{max} = 2{,}850$ K, determined by the lowest temperature (the temperature of the $T_1$ stream, 300 K) and the highest temperature (the adiabatic flame temperature, 2,700 K) respectively. This promotes physically-realizable temperature fields during the calculations.  Species limiters are not included for results presented in this section. ROMs solved via an explicit time integrator use an explicit 4-stage Runge--Kutta method. ROMs solved via an implicit time integrator use the second-order accurate backwards differentiation formula. It can be readily seen that all the ROMs using Galerkin projection method are unstable. LSPG projection generally generates ROMs which are more stable than those using Galerkin projection, though most of the LSPG-N ROMs are still unstable with increased trial basis mode count. The LSPG-C ROMs are stabilized as more trial basis modes are included, but produce more than 10\% error on average. On the other hand, the SP-LSVT ROMs are all stable (even with only 4 modes) and exhibit good error convergence with increased mode count.  %The results indicate that preserving the structure of the FOM governing equations, which is guaranteed by the SP-LSVT ROM formulation, is important in ensuring ROM robustness and accuracy.

The comparisons between the Galerkin and LSPG ROMs are consistent with the observations made by Carlberg et al.~\cite{CarlbergConsvLSPG}. However, it should be pointed out that, unlike LSPG projection which requires an implicit time integrator, the SP-LSVT ROM formulation is also applicable to explicit time integrators. Further, SP-LSVT ROMs using an explicit time integrator perform similarly to those using an implicit time integrator, as can be seen from Fig.~\ref{2d:rom_recon_err}. This allows for more flexibility and more importantly, opens possibilities for further computational efficiency enhancements by using explicit schemes over implicit schemes.

\subsubsection{Linear Stability}
\label{2d:LinearStability}
Linear stability of the various ROMs is assessed by investigating the system matrix ($\mathbf{C}$) of the linearized ROM  defined in~\ref{appendix:ROMJacobMatrix}, which describes the update  of the ROM state ($\mathbf{q}_r$)
\begin{equation}
    \mathbf{q}_r^{\iterIdx} = \mathbf{C} \mathbf{q}_r^{\iterIdx-1}.
    \label{rom:Cmatrix}
\end{equation}
If $\left\|\mathbf{C}\right\|_2 = \sigma_{\text{max}}(\mathbf{C}) \leq 1$, the linearized ROM system is considered asymptotically stable; otherwise, it is linearly unstable. 

The singular values ($\sigma_k$) of the matrix $\mathbf{C}$ are computed at each time step of the ROM calculations. The maximum singular values ($\sigma_\text{max}$) are shown for different methods (Galerkin, LSPG and SP-LSVT) and time integration schemes (explicit and implicit)  in Fig.~\ref{2d:rom_singular_value}. Due to the wide range of values spanned by $\sigma_\text{max}$, Figs.~\ref{2d:rom_sigma_Imp} (left) and ~\ref{2d:rom_sigma_Exp} (left) show a wide range for consistent comparisons between all methods. Smaller ranges of y-axis centered around 1.0 are highlighted in Figs.~\ref{2d:rom_sigma_Imp} (right) and ~\ref{2d:rom_sigma_Exp} (right). 

As can be readily seen in Fig.~\ref{2d:rom_singular_value}, all the Galerkin ROMs (Galerkin-N and Galerkin-C) are unstable (indicated in Fig.~\ref{2d:rom_recon_err} as well) with the ROM calculations terminated before the end of the training time period (27 $ms$) with  $\sigma_\text{max} > 1$ for a large portion of the calculations, which is a direct indicator of  instability. Though the LSPG-N method enables the ROM to complete the calculation spanning the entire 1.0 $ms$ training time period, the accuracy of the resulting ROM is poor as seen in Fig.~\ref{2d:rom_recon_err}. This  can be attributed to the instability indicated by the high $\sigma_\text{max} > O(10^3)$. The LSPG-C ROM shows more reasonable $\sigma_\text{max}$ values and produces stable ROMs with acceptable accuracy, but $\sigma_\text{max}$ remains higher than 1.0 during the entire 1.0 $ms$ training time period. As a consequence, the  the accuracy of the resulting ROM is contaminated as seen in Fig.~\ref{2d:rom_recon_err}. On the other hand, both implicit and explicit SP-LSVT ROMs exhibit significant improvement compared to Galerkin and LSPG ROMs with $\sigma_\text{max} \approx 1.0$, and remaining below 1.0 for most of the training period. It is of course recognized that in these highly non-linear problems, stability based on linearized systems should be considered as one (and possibly imprecise) indicator.
%Consequently, evolution with $\sigma_\text{max} > 1.0$ based on the linear stability analysis, the nonlinear ROM system can still remain numerically stable.

\begin{figure}
     \centering
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=0.9\textwidth]{./figures/SingularValueCmp_Implicit.png}
         \caption{Implicit Scheme}
         \label{2d:rom_sigma_Imp}
     \end{subfigure}
     
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=0.9\textwidth]{./figures/SingularValueCmp_Explicit.png}
         \caption{Explicit Scheme}
         \label{2d:rom_sigma_Exp}
     \end{subfigure}
     
     \caption{Linear stability comparisons based on the maximum singular values ($\sigma_{max}$) of ROM Jacobian matrices between Galerkin, LSPG and SP-LSVT ROMs with different time integration schemes for the 2D reacting  injector simulation.}\label{2d:rom_singular_value}
\end{figure}

Furthermore, the stiffness of the system matrix ($\mathbf{C}$) is investigated  by assessing the condition number ($\kappa$) defined as $\kappa \triangleq \sigma_{max} / \sigma_{min}$. The condition numbers $\kappa$ are calculated at each time step for different ROM methods. The highest ($\kappa_{max}$) and lowest ($\kappa_{min}$) condition numbers are compared between Galerkin, LSPG and SP-LSVT and summarized in Table~\ref{table:2D_condition_number}. It can be readily seen that the SP-LSVT ROM formulation results in nearly optimal conditioning. LSPG-C and Galerkin-C (Explicit Scheme) methods also produce well-conditioned systems. Unsurprisingly, the Galerkin-C ROM with an explicit scheme is unstable as indicated in Figs.~\ref{2d:rom_recon_err} and~\ref{2d:rom_sigma_Exp}. LSPG-N, Galerkin-N and Galerkin-C (Implicit Scheme) techniques are seen to generate extremely ill-conditioned matrices 
($\kappa \approx O(10^{12})$). %Such high stiffness in dynamical systems can lead to challenging numerical stability issues for ROM construction.

\begin{table}
\centering
\begin{tabular}{lll} 
\toprule
ROM Method & $\kappa_{max}$ & $\kappa_{min}$ \\
\midrule
LSPG-N & $O(10^{4})$ & $1.28$ \\ 
Galerkin-N (Explicit Scheme) & $O(10^{6})$ & $4.17$ \\ 
Galerkin-N (Implicit Scheme) & $O(10^{10})$ & $1.28$ \\ 
LSPG-C & $2.0$ & $1.21$ \\ 
Galerkin-C (Explicit Scheme) & $1.8$ & $1.75$ \\ 
Galerkin-C (Implicit Scheme) & $O(10^{12})$ & $1.25$\\ 
SP-LSVT (Explicit Scheme) & $1.3$ & $1.15$ \\
SP-LSVT (Implicit Scheme) & $1.1$ & $1.05$ \\
\bottomrule
\end{tabular}
\caption{\label{table:2D_condition_number} Comparisons of highest condition numbers of the system matrix $\mathbf{C}$ with different time integration schemes for the 2D reacting injector.}
\end{table}

As an additional {\em indicator},  the eigenvalues ($\lambda$) of the matrix $\mathbf{C}$ are  displayed in Fig.~\ref{2d:rom_eigen_value}, with the solid black line depicting the unit circle. %It should be pointed out that if $\left\|\mathbf{C}\right\|_2<1.0$, then the moduli of eigenvalues ($|\lambda|$) is less than 1.0. Therefore, whether all the eigenvalues ($\lambda$) are located within the unit circle (centered at the origin) on the complex plane (solid black line in Fig.~\ref{2d:rom_eigen_value}) is the indication of the ROM system's linear stability.  
It can be seen in Figs.~\ref{2d:rom_eigen_GvLSPG-N} and~\ref{2d:rom_eigen_GvLSPG-C} that eigenvalues exist outside the unit circle for the both Galerkin and LSPG methods, although switching from non-conservative (Galerkin-N and LSPG-N) to conservative (Galerkin-C and LSPG-C) variables does improve the linear stability. On the other hand, SP-LSVT ROMs indicate a stable behavior.  Overall, the analysis based on singular values and eigenvalues show consistent linear stability and conditioning improvements using SP-LSVT method over Galerkin and LSPG methods. 

\begin{comment}
{\color{blue}In addition, the eigenvalues $\lambda$ determine the conditions of the Jacobian matrix $\mathbf{L}$ (or the stiffness of the dynamical system), which can be directly measured by the condition number $\kappa$ defined as $\kappa = |\lambda|_{max} / |\lambda|_{min}$ with $|\cdot|$ representing the moduli of $\lambda$. The condition numbers $\kappa$ are calculated at each time step for different ROM methods. The order of magnitudes of the highest condition numbers $\kappa_{max}$ are compared between Galerkin, LSPG and SP-LSVT and summarized in Table~\ref{table:2D_condition_number}. It can be readily seen that the SP-LSVT ROM method produces Jacobian matrices with good condition numbers, less then 20, indication of non-stiff system. However, both the Galerkin-C and LSPG-C methods generate stiffer ROM system with Jacobian matrices of condition numbers higher than 200 while the condition numbers increase higher than 4000 and produce extremely stiff system with ill-conditioned Jacobian matrices if Galerkin-N and LSPG-N methods are used. It is well-recognized that the ill-conditioned Jacobian matrices can lead to challenging numerical stiffness.}

\begin{figure}
     \centering
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=0.7\textwidth]{./figures/EigenValueCmp_GvLSPG-N.png}
         \caption{Galerkin-N and LSPG-N}
         \label{2d:rom_eigen_GvLSPG-N}
     \end{subfigure}
     
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=0.7\textwidth]{./figures/EigenValueCmp_GvLSPG-C.png}
         \caption{Galerkin-C and LSPG-C}
         \label{2d:rom_eigen_GvLSPG-C}
     \end{subfigure}
     
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=0.35\textwidth]{./figures/EigenValueCmp_LSPG-VT.png}
         \caption{SP-LSVT}
         \label{2d:rom_eigen_LSPT-VT}
     \end{subfigure}
     \caption{ROM eigenvalues comparisons between Galerkin, LSPG and SP-LSVT ROMs with different time integration schemes for the 2D reacting single injector simulation.}\label{2d:rom_eigen_value}
\end{figure}
\end{comment}

\begin{figure}
     \centering
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=1.0\textwidth]{./figures/CmatrixEigenValueCmp_GvLSPG-N.png}
         \caption{Galerkin-N and LSPG-N}
         \label{2d:rom_eigen_GvLSPG-N}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=1.0\textwidth]{./figures/CmatrixEigenValueCmp_GvLSPG-C.png}
         \caption{Galerkin-C and LSPG-C}
         \label{2d:rom_eigen_GvLSPG-C}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=1.0\textwidth]{./figures/CmatrixEigenValueCmp_LSPG-VT.png}
         \caption{SP-LSVT}
         \label{2d:rom_eigen_LSPT-VT}
     \end{subfigure}
     \caption{Linear stability comparisons based on eigenvalues ($\lambda$) of ROM Jacobian matrices between Galerkin, LSPG and SP-LSVT ROMs with different time integration schemes for the 2D reacting  injector simulation.}\label{2d:rom_eigen_value}
\end{figure}

\subsubsection{Time Step Size Sensitivity}
The sensitivity of the SP-LSVT ROMs to the physical time step size is evaluated at four different time step sizes, $\dt_\text{ROM} \in \{ \dt_\text{FOM}, 2\dt_\text{FOM}$, $5\dt_\text{FOM}$, $10\dt_\text{FOM}\}$. The reconstruction error, as defined in Eq.~\ref{rom:reconstr_err}, is evaluated for both explicit and implicit time integration schemes. The results are shown in Fig.~\ref{2d:rom_recon_err_onDt}, displaying largely overlapping plots. Changing the time-step has a very minor impact on the solutions integrated with an implicit scheme and an even smaller effect on those integrated with an explicit scheme. Using an explicit time integration scheme, setting the physical time step to ten times that of the FOM ($\dt_\text{ROM} = 10\dt_\text{FOM}$) gives essentially identical reconstruction error to that of a ROM using the same physical time step as the FOM ($\dt_\text{ROM} = \dt_\text{FOM}$). With an implicit time integration scheme, minor differences show that the ROM solutions with a larger time step ($\dt_\text{ROM} = 5\dt_\text{FOM}$ and $10 \dt_\text{FOM}$) are marginally less accurate. The results in Fig.~\ref{2d:rom_recon_err_onDt} indicate that the SP-LSVT ROMs are not as sensitive to the time step size as one might expect from the analysis by Carlberg et al.~\cite{Carlberg2017}, which showed that LSPG ROMs achieve optimal accuracy at intermediate time step sizes. Such a sensitivity to the time step size for LSPG ROMs is also observed in the current test problem, as shown in Fig.~\ref{2d:lspgC_rom_recon_err_onDt} for LSPG-C ROMs, which are identified to be the most stable method among the Galerkin and LSPG ROMs. Using a time step size of $\dt_\text{ROM} = 2\dt_\text{FOM}$ in the LSPG-C ROMs helps stabilize the unstable ROMs and improves their accuracy, but become less accurate as the time step increases to $5\dt_\text{FOM}$ and $10\dt_\text{FOM}$. This sensitivity to time step in the least-squares formulation does not appear to be a significant issue for the SP-LSVT method, an aspect that requires further investigation and analysis. 
%An issue that may be a factor in the present results is that implicit time integration schemes require the calculation of Jacobians from the ROM-reconstructed solutions. It is possible that accuracy may be impacted not only by the truncation of POD modes (i.e. loss of small-scale dynamics) but also by errors in the computed Jacobians. In general, Jacobian calculations are more challenging for reacting flow simulations with stiff chemical kinetics, and these errors may escalate in regions where the solution strays from the original calculation. 

%The less sensitivity of SP-LSVT ROMs to time step indicates the capability of ROMs in providing consistent modeling fidelity, even when larger time steps are used, thereby producing improved computational efficiency.
 
\begin{figure}
	\centering
	\includegraphics[width=0.8\textwidth]{./figures/2d_rom_recon_errorOnDt.png}
	\caption{Sensitivity of SP-LSVT ROMs to physical time step size for both explicit and implicit time integration schemes for the 2D reacting  injector simulation.}\label{2d:rom_recon_err_onDt} 
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.4\textwidth]{./figures/2d_lspgQc_rom_recon_errorOnDt.png}
	\caption{Sensitivity of LSPG-C ROMs with implicit time integration to physical time step size for the 2D reacting  injector simulation.}\label{2d:lspgC_rom_recon_err_onDt} 
\end{figure}

\subsubsection{SP-LSVT ROM Enhancement with Species Limiters}
\label{sec:2d_limiters}
It has been demonstrated in Fig.~\ref{2d:rom_recon_err} that the SP-LSVT ROMs are able to accurately reproduce the FOM solutions (i.e. pressure, velocities, temperature and species mass fraction fields) with approximately 3\% error using 100 trial basis modes. We now evaluate the ability of the ROM in representing the heat release rate, an important quantity of interest for reacting flow problems. 

\begin{figure}
	\centering
	\includegraphics[width=0.8\textwidth]{./figures/HeatReleaseCmp_FOMvsROM_noSpecLimiter.png}
	\caption{Comparisons of unsteady heat release rate field at representative time instances between FOM and SP-LSVT 100-mode ROM with temperature limiter only.}\label{2d:q_cmp_FOMvsLSPGVTROM_noSpecLimiter} 
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.8\textwidth]{./figures/YO2Cmp_FOMvsROM_noSpecLimiter.png}
	\caption{Comparisons of \oxygen\ mass fraction field at representative time instances between FOM and SP-LSVT 100-mode ROM with temperature limiter only.}\label{2d:O2_cmp_FOMvsLSPGVTROM_noSpecLimiter} 
\end{figure}

Comparisons of the instantaneous heat release rate fields at three different time instances are shown in Fig.~\ref{2d:q_cmp_FOMvsLSPGVTROM_noSpecLimiter}. The SP-LSVT ROM uses 100 trial basis modes, solved using the explicit time integration scheme, and applies the temperature limiter with bounds $T_{min} = 270$ K and $T_{max} = 2{,}850$ K. The species limiter introduced in Section~\ref{limiters} is not yet applied for this simulation. It is seen that the reconstruction of the heat release rate  is very inaccurate with  excessive burning occurring within the recirculation region. Such errors can usually be attributed to the spurious oscillations in species mass fractions near sharp gradients in the species mass fraction field. Figure~\ref{2d:O2_cmp_FOMvsLSPGVTROM_noSpecLimiter} compares the \oxygen\ mass fraction field between the FOM and ROM at the same time instances in Fig.~\ref{2d:q_cmp_FOMvsLSPGVTROM_noSpecLimiter}. The contour levels of the \oxygen\ mass fraction field are selected to be in log scale to highlight the presence of these small magnitude ($<$ 0.1\%) spurious oscillations in the ROM. These are concentrated within the recirculation region and coincide with the excessive heat release rate (Fig.~\ref{2d:q_cmp_FOMvsLSPGVTROM_noSpecLimiter}). 

Interestingly, the spurious oscillations in the \oxygen\ mass fraction field and the resulting excessive burning did not make the ROM unstable in this case, and the ROM can still provide a reasonable representation of the solution variables (pressure, velocities, temperature and species mass fractions). However, the ability of the ROM to represent the heat release rate is  lacking.  Therefore, the species limiter introduced in Eq.~\ref{rom:species_limiter_nonpremixed} is applied to the SP-LSVT 100-mode ROM here with $T_{th} = 2{,}200$ K (80\% of the adiabatic flame temperature, $T_{ad}$) and $\delta = 1 \times 10^{-5}$. The resulting flow field snapshots, shown in Fig.~\ref{2d:qO2_cmp_FOMvsLSPGVTROM_SpecLimiter}, display significant improvements in representing the heat release rate. It can be readily seen that most of the spurious oscillations in Fig.~\ref{2d:O2_cmp_FOMvsLSPGVTROM_noSpecLimiter} have been eliminated by the species limiter, which yields a significantly more accurate representation of the heat release rate compared to Fig.~\ref{2d:q_cmp_FOMvsLSPGVTROM_noSpecLimiter}. The species limiter proves to be effective and necessary in enabling the ROM to provide an accurate representation of important features in reacting flow problems (e.g. heat release rate and flame propagation speed) as also illustrated in~\ref{appendix:species_oscillations}. 

\begin{figure}
	\centering
	\includegraphics[width=0.8\textwidth]{./figures/HeatReleaseO2Cmp_FOMvsROM_SpecLimiter.png}
	\caption{Unsteady heat release rate and $\text{O}_2$ mass fraction fields at representative time instances for SP-LSVT 100-mode ROM with temperature and species limiters.}\label{2d:qO2_cmp_FOMvsLSPGVTROM_SpecLimiter} 
\end{figure}



==> figures/results_3DSingleInjector.tex <==
\subsection{3D Reacting  Injector}
\label{3d:injector}
Next, we extend the investigations to a  3D representation of the generic laboratory-scale single injector combustor~\cite{YuJPP}. The configuration is shown in Fig.~\ref{3d:geometry}. Similar to the 2D case in Section~\ref{2d:injector}, the 3D problem consists of a shear coaxial injector with an outer passage, $T_1$, that introduces fuel (100\% \methane\ at 300 K) near the downstream end of the coaxial center passage, $T_2$, that feeds oxidizer (42\% gaseous \oxygen\ by mass and 58\% gaseous \water\ by mass at 660 K) to the combustion chamber. 

\begin{figure}
	\centering
	\includegraphics[width=0.8\textwidth]{./figures/3d_geometry.png}
	\caption{Computational configuration of 3D reacting  injector.}\label{3d:geometry} 
\end{figure}

The operating conditions for this 3D reacting flow simulation are maintained similar to the conditions in the laboratory combustor~\cite{YuJPP,YuPhD}, with an adiabatic flame temperature of approximately 2,600 K and a mean chamber pressure of 1.1 MPa. The $T_1$ and $T_2$ streams are both fed with constant mass flow rates: 0.027 kg/s and 0.32 kg/s, respectively. As in the 2D case, a non-reflective boundary condition is enforced at the downstream outflow boundary. A sinusoidal pressure perturbation (with amplitude 5\% of the mean pressure) at 4,000 Hz is imposed at this boundary. Different from the finite rate global reaction model used for the 2D problem, combustion is represented by the flamelet progress variable (FPV) model~\cite{Pierce2004_FPV} with more detailed chemical kinetics, GRI-1.2~\cite{GRI_12}, which consists of 32 species and 177 chemical reactions. The chemical species are treated as thermally perfect gases. Note that although 32 chemical species are modeled, the FPV model only solves transport equations for three scalar quantities: the mean mixture fraction (${Z}_{mean}$), the mixture fraction variance (${Z''^2}$), and the reaction progress variable (${C}_{mean}$) as described in~\ref{appendix:fom_eq}. Individual chemical species mass fractions are looked up from pre-computed flamelet manifolds~\cite{FlameletJointPDFModel}.

\begin{figure}
	\centering
	\includegraphics[width=0.8\textwidth]{./figures/3d_fom_snapshots.png}
	\caption{Representative instantaneous snapshots of pressure (top) and temperature (bottom) fields from FOM simulation of the 3D reacting  injector.}\label{3d:fom_snapshots} 
\end{figure}

The 3D FOM is solved using the second-order accurate backwards differentiation formula and dual time-stepping, with a constant physical time step size of 1.0 $\mu$s. The computational mesh is composed of a total of 589,395 finite volume cells, resulting in a total of 4,715,160 degrees of freedom. A representative instantaneous snapshot is shown in Fig.~\ref{3d:fom_snapshots}. Similar to the 2D solutions in Fig.~\ref{2d:fom_snapshots}, the pressure exhibits global dynamics while the combustion dynamics, characterized by temperature, show more local convection-dominated features. However, due to the improved modeling of mixing in 3D simulations, the combustion dynamics exhibit more coherent structures than in the 2D case where the dynamics are more intermittent. Solution snapshots are stored at every physical time step over a time duration of 1.0 ms, corresponding to a total of 1,000 snapshots. All snapshots are used to generate POD bases for ROM construction.

\subsubsection{POD and ROM Characteristics}
\label{3d:results-pod_rom}

The characteristics of the POD bases and ROMs are evaluated based on the POD residual energy (Eq.~\ref{pod:res_energy}) and ROM reconstruction error (Eq.~\ref{rom:reconstr_err}), shown in Fig.~\ref{3d:romErr_podEnergy}. The POD residual energy still shows a relatively slow decay similar to the 2D case (Fig.~\ref{2d:pod_res_energy}). More than 43 POD modes are required to retrieve 99\% of the energy, and 100 POD modes are required to retrieve 99.9\%. ROMs are constructed using the SP-LSVT formulation with either the explicit four-stage Runge--Kutta method or the implicit second-order accurate backwards differentiation formula.  The temperature limiter ($T_{min} = 270$ K and $T_{max} = 2{,}800$ K), determined by the temperature of the $T_1$ stream (300 K), and the adiabatic flame temperature ($2,600$ K). In addition, species limiters ($T_{th} = 2{,}500$ K, $C_\text{ref} = 0.85$, $Z_\text{st} = 0.096$, $\delta = 1\times 10^{-5}$) are applied during the SP-LSVT ROM calculations to ensure reasonable modeling of the heat release rate. 
It can be readily seen in Fig.~\ref{3d:romErr_podEnergy} that all SP-LSVT ROMs are stable using both explicit and implicit time integration schemes.  Less than 3\% $L^2$ error can be reached by using more than 40 POD trial basis modes.

\begin{figure}
	\centering
	\includegraphics[width=0.6\textwidth]{./figures/3d_rom_recon_error_and_pod_energy.png}
	\caption{Global ROM reconstruction error for SP-LSVT method with different time integration schemes and POD residual energy distribution for the 3D reacting  injector simulation.}\label{3d:romErr_podEnergy} 
\end{figure}

\subsubsection{Hyper-reduction}\label{3d:injector_hyperReduction}
In this section, we extend the investigations to SP-LSVT ROMs with hyper-reduction, as introduced in Section~\ref{hyper_reduction}, to achieve enhancement in computational efficiency. %Instead of evaluating the non-linear function $\mathbf{r}$ and the test basis $\mathbf{\hat{W}}^n$ in Eq.~\ref{rom:lspg_proj} at each mesh point of the computation domain, they are evaluated only at sampled mesh points through the DEIM formulation in Eq.~\ref{rom:lspg_proj_deim}.
As mentioned previously, the rank-revealing QR factorization and randomized oversampling~\cite{PeherstorferODEIM} are used to determine the selection of the mesh points. Figure~\ref{3d:rom_sampling} displays sampled cells of the two sparse sampled meshes investigated here, alongside the fully-sampled mesh.

\begin{figure}
	\centering
	\includegraphics[width=0.7\textwidth]{./figures/3d_sampled_mesh.png}
	\caption{Comparisons of sampled meshes for the 3D reacting  injector simulation.}\label{3d:rom_sampling} 
\end{figure}

The hyper-reduced SP-LSVT ROMs are evaluated based on their accuracy (reconstruction error) and computational efficiency. Computational efficiency is measured by both wall clock time (real-world time to complete the simulation) and CPU time (wall clock time multiplied by the number of computational cores used). The FOM computations were performed on 4 compute nodes (two Haswell CPUs @ 2.60GHz per node, 20 cores per node) and 128 GB of RAM. The training data generation required approximately  710 core-hours, to simulate 1 ms (1,000 snapshots). Results using the explicit time integrator and implicit time integrator are displayed in Table~\ref{table:3D_hyperreduction_exp} and Table~\ref{table:3D_hyperreduction_imp}, respectively, for three different physical time step sizes. Computational efficiency results are reported as the ratio of the FOM computational time to the ROM computational time.

%{\color{red}There is no explanation of why the DEIM results are often MORE accurate than the full ROM results.}

It can be readily seen that the reconstruction errors for the hyper-reduced ROMs are similar to that of the unsampled ROM. All SP-LSVT ROMs achieve a reconstruction error below 2.5\% using the explicit time integration scheme, and the hyper-reduced ROMs lead to greatly improved efficiency with fewer sampled degrees of freedom and larger physical time steps. This does not seem to affect the accuracy of the explicit SP-LSVT ROMs, consistent with the observations for the 2D case in Fig.~\ref{2d:rom_recon_err_onDt}. However, the reconstruction errors from implicit SP-LSVT ROMs are sensitive to the physical time steps, with error increasing with the time step. A possible contributing factor to the sensitivity of implicit SP-LSVT ROMs to the physical time steps is that implicit time integration schemes require the calculation of Jacobians from the ROM-reconstructed solutions. It is possible that accuracy may be impacted not only by the truncation of trial basis modes (i.e. loss of small-scale dynamics) but also by errors in the computed Jacobians. In general, Jacobian calculations are more challenging for extremely stiff reacting flow simulations, and these errors may escalate in regions where the solution deviates from the original calculation when a larger physical time step is used.

It should be pointed out that even without hyper-reduction, a larger time step and explicit time integration scheme can already achieve $> O(20)$ acceleration in wall clock and CPU times. With hyper-reduction, more than a factor of $O(300)$ improvement in wall clock time and a factor of $O(600)$ improvement in CPU time can be achieved with an explicit time integration scheme and a physical time step 10 times that of the FOM, producing less than 2\% reconstruction error.

\begin{table}
\centering
\begin{tabular}{lllll} 
\toprule
Time Step Ratio & Mesh & $\epsilon$ & Wall Clock Time Ratio & CPU Time Ratio \\
\midrule
\multirow{3}{1em}{1.0} & Full Mesh (100\%) & $2.0 \times 10^{-2}$ & 2.6 & 2.6 \\
& Sampled Mesh (10\%) & $1.3 \times 10^{-2}$ & 7.3 & 7.3 \\
& Sampled Mesh (1\%) & $1.5 \times 10^{-2}$ & 32.1 & 64.3 \\
\midrule
\multirow{3}{1em}{5.0} & Full Mesh (100\%) & $1.9 \times 10^{-2}$ & 13.1 & 13.1 \\
& Sampled Mesh (10\%) & $1.8 \times 10^{-2}$ & 37.1 & 37.1 \\
& Sampled Mesh (1\%) & $2.3 \times 10^{-2}$ & 161.8 & 323.6 \\
\midrule
\multirow{3}{1em}{10} & Full Mesh (100\%) & $1.6 \times 10^{-2}$ & 26.2 & 26.2 \\
& Sampled Mesh (10\%) & $1.4 \times 10^{-2}$ & 71.7 & 71.7 \\
& Sampled Mesh (1\%) & $1.6 \times 10^{-2}$ & 319.0 & 638.0 \\
\bottomrule
\end{tabular}
\caption{\label{table:3D_hyperreduction_exp} Summary of global ROM reconstruction error, wall clock time and CPU time ratios of the hyper-reduced SP-LSVT ROMs using explicit scheme with different number of sampling points and time steps sizes.}
\end{table}

\begin{table}
\centering
\begin{tabular}{lllll} 
\toprule
Time Step Ratio & Mesh & $\epsilon$ & Wall Clock Time Ratio & CPU Time Ratio \\
\midrule
\multirow{3}{1em}{1.0} & Full Mesh (100\%) & $2.2 \times 10^{-2}$ & 1.8 & 1.8 \\
& Sampled Mesh (10\%) & $1.5 \times 10^{-2}$ & 5.8 & 5.8 \\
& Sampled Mesh (1\%) & $1.6 \times 10^{-2}$ & 24.7 & 49.5 \\
\midrule
\multirow{3}{1em}{5.0} & Full Mesh (100\%) & $6.2 \times 10^{-2}$ & 4.5 & 4.5 \\
& Sampled Mesh (10\%) & $4.2 \times 10^{-2}$ & 27.6 & 27.6 \\
& Sampled Mesh (1\%) & $3.8 \times 10^{-2}$ & 124.5 & 249.0 \\
\midrule
\multirow{3}{1em}{10} & Full Mesh (100\%) & $8.0 \times 10^{-2}$ & 9.0 & 9.0 \\
& Sampled Mesh (10\%) & $7.0 \times 10^{-2}$ & 56.7 & 56.7 \\
& Sampled Mesh (1\%) & $6.6 \times 10^{-2}$ & 249.3 & 498.7 \\
\bottomrule
\end{tabular}
\caption{\label{table:3D_hyperreduction_imp} Summary of global ROM reconstruction error, wall clock time and CPU time ratios of the hyper-reduced SP-LSVT ROMs using implicit scheme with different number of sampling points and time steps sizes.}
\end{table}

\begin{comment}
\begin{table}
\centering
\begin{tabular}{ |c|c|c|c|c| } 
\hline
Time Step Ratio & Mesh & $\epsilon$ & Wall Clock Time Ratio & CPU Time Ratio \\
\hline
\multirow{3}{1em}{1.0} & Full Mesh (100\%) & $2.0 \times 10^{-2}$ & 2.6 & 2.6 \\
& Sampled Mesh (10\%) & $1.3 \times 10^{-2}$ & 7.3 & 7.3 \\
& Sampled Mesh (1\%) & $1.5 \times 10^{-2}$ & 32.1 & 64.3 \\
\hline
\multirow{3}{1em}{5.0} & Full Mesh (100\%) & $1.9 \times 10^{-2}$ & 13.1 & 13.1 \\
& Sampled Mesh (10\%) & $1.8 \times 10^{-2}$ & 37.1 & 37.1 \\
& Sampled Mesh (1\%) & $2.3 \times 10^{-2}$ & 161.8 & 323.6 \\
\hline
\multirow{3}{1em}{10} & Full Mesh (100\%) & $1.6 \times 10^{-2}$ & 26.2 & 26.2 \\
& Sampled Mesh (10\%) & $1.4 \times 10^{-2}$ & 71.7 & 71.7 \\
& Sampled Mesh (1\%) & $1.6 \times 10^{-2}$ & 319.0 & 638.0 \\
\hline
\end{tabular}
\caption{\label{table:3D_hyperreduction_exp} Summary of global ROM reconstruction error, wall clock time and CPU time ratios of the hyper-reduced SP-LSVT ROMs using explicit scheme with different number of sampling points and time steps.}
\end{table}

\begin{table}
\centering
\begin{tabular}{ |c|c|c|c|c| } 
\hline
Time Step Ratio & Mesh & $\epsilon$ & Wall Clock Time Ratio & CPU Time Ratio \\
\hline
\multirow{3}{1em}{1.0} & Full Mesh (100\%) & $2.2 \times 10^{-2}$ & 1.8 & 1.8 \\
& Sampled Mesh (10\%) & $1.5 \times 10^{-2}$ & 5.8 & 5.8 \\
& Sampled Mesh (1\%) & $1.6 \times 10^{-2}$ & 24.7 & 49.5 \\
\hline
\multirow{3}{1em}{5.0} & Full Mesh (100\%) & $6.2 \times 10^{-2}$ & 4.5 & 4.5 \\
& Sampled Mesh (10\%) & $4.2 \times 10^{-2}$ & 27.6 & 27.6 \\
& Sampled Mesh (1\%) & $3.8 \times 10^{-2}$ & 124.5 & 249.0 \\
\hline
\multirow{3}{1em}{10} & Full Mesh (100\%) & $8.0 \times 10^{-2}$ & 9.0 & 9.0 \\
& Sampled Mesh (10\%) & $7.0 \times 10^{-2}$ & 56.7 & 56.7 \\
& Sampled Mesh (1\%) & $6.6 \times 10^{-2}$ & 249.3 & 498.7 \\
\hline
\end{tabular}
\caption{\label{table:3D_hyperreduction_imp} Summary of global ROM reconstruction error, wall clock time and CPU time ratios of the hyper-reduced SP-LSVT ROMs using implicit scheme with different number of sampling points and time steps.}
\end{table}
\end{comment}

% \begin{figure}
% 	\centering
%     \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=0.6\textwidth]{./figures/3d_rom_acceleration-rk4-WallClock.png}
%          \caption{SP-LSVT (Explicit Scheme)}
%           \label{3d:SP-LSVTExp-wallclock}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=0.6\textwidth]{./figures/3d_rom_acceleration-rk4-WallClock.png}
%          \caption{SP-LSVT (Implicit Scheme) \color{red}{to be updated}}
%           \label{3d:SP-LSVTImp-wallclock}
%     \end{subfigure}
% 	\caption{Global ROM reconstruction error of the hyper-reduced SP-LSVT ROMs compared against acceleration in \emph{wall clock time} with different number of sampling points (decreasing along the x-axis), time steps and time integration schemes. \color{red}{to be updated with load-balancing}}\label{3d:rom_acceleration_wallclock} 
% \end{figure}
% \begin{figure}
% 	\centering
%     \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=0.6\textwidth]{./figures/3d_rom_acceleration-rk4-CPUTime.png}
%          \caption{SP-LSVT (Explicit Scheme)}
%           \label{3d:SP-LSVTExp-cpu}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=0.6\textwidth]{./figures/3d_rom_acceleration-rk4-CPUTime.png}
%          \caption{SP-LSVT (Implicit Scheme) \color{red}{to be updated}}
%           \label{3d:SP-LSVTImp-cpu}
%     \end{subfigure}
% 	\caption{SP-LSVT ROM acceleration in \emph{CPU time} with hyper-reduction with different number of sampling points (decreasing along the x-axis), time steps and time integration schemes. \color{red}{to be updated with load-balancing}}\label{3d:rom_acceleration_cpu} 
% \end{figure}

\subsubsection{Evaluations of Future-state Prediction Capabilities}
The final evaluation is performed on the ability of the SP-LSVT ROMs to provide future-state predictions beyond the 1.0 ms training duration used to compute the POD trial bases. The evaluation is performed for SP-LSVT ROMs using 60 trial basis modes and an explicit time integration scheme. ROMs are constructed with and without hyper-reduction, where the hyper-reduced ROM uses the 1\% sampled mesh shown in Fig.~\ref{3d:rom_sampling}. All ROMs are computed with a time step ten times that of the FOM time step. The accuracy is quantified and evaluated based on the ROM error in representing the $\varIdx^{th}$ physical quantity (e.g. $p, \mathbf{u}, T, Y_j$), estimated at each time step, $n$, defined in two levels. First, the ROM error is evaluated based on the projected FOM solutions as follows:
 \begin{equation}
    \tilde{\epsilon}^{n}_{\varIdx} = \frac{\left\|\mathbf{\tilde{q}}^n_{p,\varIdx}-\mathbf{\tilde{q}}^n_{p,\text{pod},\varIdx}\right\|_2}{\left\|{\mathbf{\tilde{q}}^n_{p,\text{pod},\varIdx}}\right\|_2},
    \label{rom:proj_err_onProjFOM}
\end{equation}
where $\mathbf{\tilde{q}}^\iterIdx_{p,\varIdx}$ represents the $i^{th}$ solution variable of the state vector, $\mathbf{\tilde{q}}^\iterIdx_{p}$, at time step $n$ from ROM simulations following Eq.~\ref{pod:expansion_qp}. We define $\mathbf{\tilde{q}}^n_{p,\text{pod},\varIdx}$ to represent the $i^{th}$ solution variable of the state vector, $\mathbf{\tilde{q}}^\iterIdx_{p,\text{pod}}$, at time step $n$ evaluated as, $\mathbf{\tilde{q}}^\iterIdx_{p,\text{pod}}= \mathbf{q}_{p,ref} + \mathbf{H}^{-1}\mathbf{\hat{V}} \mathbf{\hat{V}}^T \mathbf{q}^n_{p}$. similar to Eq.~\ref{pod:expansion_qp}. This is referred to as the projected FOM solution.


The ROM error (with respect to the projected FOM solutions) in the pressure ($\varIdx=1$ in Eq.~\ref{rom:proj_err_onProjFOM}) and temperature ($\varIdx=5$ in Eq.~\ref{rom:proj_err_onProjFOM}) fields are compared in Fig.~\ref{3d:rom_future_prjErronPOD} within the training period ($\timeVar = [25, 26]$ ms) and beyond -- labeled as the testing period ($\timeVar = (26,30]$ ms). Within the training period, the ROMs are able to track the projected FOM solutions for both pressure and temperature accurately (well below 1\% error for pressure and well below 4\% error for temperature). Beyond the training period, however, the error start to increase noticeably. In the testing period, error in the pressure field is still well below 2\% error, which indicates good accuracy of the ROMs in matching the projected pressure field. On the other hand, the time evolution of error in the temperature field exhibits error as high as 12\%, with large-amplitude oscillations between 4\% and 12\%. This is a particular issue for the ROM with hyper-reduction. These oscillations result in approximately 8\% error on average, which can still be considered marginally accurate given the fact that the temperature field is characterized with sharp gradients. Such sharp gradients can be challenging features to match based on $L^2$-norm error, as measured by Eq.~\ref{rom:proj_err_onProjFOM}.

\begin{figure}
	\centering
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=0.7\textwidth]{./figures/L2Norm-vs-Time_RK4_ConsvEq_onROM-p.png}
         \caption{Error \st{on} {\color{blue}in} pressure}
          \label{3d:SP-LSVT-errPonPOD}
    \end{subfigure}
    \centering
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=0.7\textwidth]{./figures/L2Norm-vs-Time_RK4_ConsvEq_onROM-T.png}
         \caption{Error \st{on} {\color{blue}in} temperature}
          \label{3d:SP-LSVT-errTonPOD}
    \end{subfigure}
	\caption{Comparisons of time evolution of errors with respect to the projected FOM solutions.}\label{3d:rom_future_prjErronPOD} 
\end{figure}

\subsubsection{Limitations of Linear Static Bases}
Though the SP-LSVT ROMs perform well in comparison to  the projected FOM solutions in both training and testing periods, it is necessary to evaluate the ROM predictions based on the truth (i.e. the FOM solutions). Therefore, the second-level evaluation bases the ROM error on the FOM solutions

\begin{equation}
    \epsilon^{n}_{\varIdx} = \frac{\left\|\mathbf{\tilde{q}}^n_{p,\varIdx}-{\mathbf{q}^n_{p,\varIdx}}\right\|_2}{\left\|{{\mathbf{q}^n_{p,\varIdx}}}\right\|_2},
    \label{rom:proj_err}
\end{equation}
%where $\mathbf{\tilde{q}}^\iterIdx_{p,\varIdx}$ represents the $i^{th}$ solution variable of the state vector, $\mathbf{\tilde{q}}^\iterIdx_{p}$,  at time step $n$ from ROM simulations following Eq.~\ref{pod:expansion_qp}.
%where $\mathbf{\hat{q}}^n_{p,\varIdx} = \mathbf{q}_{p,\varIdx,ref} + \mathbf{H}^{-1}\mathbf{\hat{V}}_{\varIdx} \mathbf{\hat{q}}^n_r$ based on Eq.~\ref{pod:expansion_qp} and $\mathbf{\hat{V}}_{\varIdx}$ is the portion of the POD basis corresponding to the $\varIdx^{th}$ physical quantity. %(e.g. if $k=1$, $\mathbf{q}_{p,k}$ represents pressure, $p$ and if $k=3$, $\mathbf{q}_{p,k}$ represents temperature, $T$).
where $\mathbf{q}^n_{p,\varIdx}$ is directly obtained from the FOM solutions. Since the error of POD-based ROM is bounded by the projection error of the POD basis, the POD projection error is quantified as a baseline
\begin{equation}
    \epsilon^{n}_{\varIdx} = \frac{\left\|\mathbf{\tilde{q}}^n_{p,\text{pod},\varIdx}-{\mathbf{q}^n_{p,\varIdx}}\right\|_2}{\left\|{{\mathbf{q}^n_{p,\varIdx}}}\right\|_2}.
    \label{rom:proj_err_pod}
\end{equation}
%where $\mathbf{\tilde{q}}^n_{p,\text{pod},\varIdx}$ represents the $i^{th}$ solution variable of the state vector, $\mathbf{\tilde{q}}^\iterIdx_{p,\text{pod}}$, at time step $n$ evaluated as, $\mathbf{\tilde{q}}^\iterIdx_{p,\text{pod}}= \mathbf{q}_{p,ref} + \mathbf{H}^{-1}\mathbf{\hat{V}} \mathbf{\hat{V}}^T \mathbf{q}^n_{p}$ similar to Eq.~\ref{pod:expansion_qp}.
%with $\mathbf{\hat{q}}^n_{p,\varIdx} = \mathbf{q}_{p,\varIdx,ref} + \mathbf{H}^{-1}\mathbf{\hat{V}}_{\varIdx} \left(\mathbf{\hat{V}}^T \mathbf{q}^n_{p}\right)$ 



%The evaluation is performed for SP-LSVT ROMs using 60 POD modes and an explicit time integration scheme. ROMs are constructed with and without hyper-reduction, where the hyper-reduced ROM uses the 1\% sampled mesh shown in Fig.~\ref{3d:rom_sampling}. All ROMs are computed with a time step ten times that of the FOM time step. %The corresponding POD projection error is also calculated as the baseline to assess the limitations for the ROM accuracy as it should be recognized that the error of POD-based ROM is bounded by the projection error of the POD basis. 

Similarly, the ROM errors (with respect to the FOM solutions in the pressure ($\varIdx=1$ in Eqs.~\ref{rom:proj_err} and~\ref{rom:proj_err_pod}) and temperature ($\varIdx=5$ in Eqs.~\ref{rom:proj_err} and~\ref{rom:proj_err_pod}) fields are compared in Fig.~\ref{3d:rom_future_prjErr}. %within the training period ($\timeVar = [25, 26]$ ms) and beyond ($\timeVar = (26,30]$ ms). 
Within the training period in which the dynamics are well-represented, as indicated by low POD projection error  ($<$ 0.25\% error for pressure and $<$ 2\% error for temperature), the ROMs are able to represent both pressure and temperature accurately ($<$ 1\% error for pressure and $<$ 5\% error for temperature), consistent with Fig.~\ref{3d:rom_future_prjErronPOD}. However, challenges arise during future-state predictions in the testing period. Though the POD trial basis and the SP-LSVT ROMs are able to reasonably represent the future-state pressure dynamics (well below 3\% error), they are unable to accurately represent the dynamics of the temperature field after the end of the training period ($\timeVar = 26$ ms). In contrast to the small error increase (from 4\% to 6\%) at $\timeVar = 26$ ms in Fig.~\ref{3d:rom_future_prjErronPOD}, there is a significant increase in error at this point, from less than 5\% to more than 20\%.  We emphasize  that this significant error increase is mainly due to the POD projection error (and not the ROM formulation), and thus reflects the insufficiency of the POD trial basis in accurately representing the system dynamics beyond the training period. 

The observed challenges in future-state projection error can be largely attributed to the chaotic nature of the dynamics as shown in Fig~\ref{3d:fom_snapshots}. The pressure field exhibits organized dynamics due to the strong forcing introduced downstream, which allows the ROMs to provide reasonable predictions in the future state as the POD trial basis generated within the training period are able to easily represent such organized dynamics. However, in turbulent reacting flows (characterized by transport of strong temperature gradients), chaotic and non-stationary features present a major  challenge. Although the basis can represent convection features within the training period, it is unable to represent features beyond the training period, and therefore produce significant errors in the ROMs. This is not a flaw in the SP-LSVT technique, but rather a limitation of using a linear and static basis set. Nevertheless, the SP-LSVT ROMs are able to provide accurate predictions of pressure dynamics, which is an important quantity of interest for reacting flow problems, especially in practical engineering applications.

\begin{figure}
	\centering
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=0.7\textwidth]{./figures/L2Norm-vs-Time_RK4_ConsvEq_onFOM-p.png}
         \caption{Error \st{on} {\color{blue}in} pressure}
          \label{3d:SP-LSVT-errP}
    \end{subfigure}
    \centering
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=0.7\textwidth]{./figures/L2Norm-vs-Time_RK4_ConsvEq_onFOM-T.png}
         \caption{Error \st{on} {\color{blue}in} temperature}
          \label{3d:SP-LSVT-errT}
    \end{subfigure}
	\caption{Comparisons of time evolution of errors with respect to the FOM solution.}\label{3d:rom_future_prjErr} 
\end{figure}

==> intro_cw.tex <==
\section{Introduction (CW)}
\label{intro}
With advances in computing architectures and \st{computational} algorithms, high-fidelity multi-physics simulations are becoming integral to the analysis and design of complex systems. A pertinent example is that of reacting flow simulations~\cite{adityaDNS, OefeleinSupercritical}, which play an important role in the investigation and understanding of combustion dynamics in propulsion systems operating at high pressures and temperatures. Such simulations provide details which cannot be quantitatively accessed through experiments. Accurate and efficient modeling of combustion dynamics in a practical environment has the potential to improve engine performance and reduce failures. However, large eddy simulations (LES) of combustion dynamics -- even for small-scale engines~\cite{UrbanoLES2016} -- typically require $O(10^7)$ CPU-hours per simulation, and are thus impractical in many-query applications such as engineering design and uncertainty quantification. In the present work, we develop model order reduction techniques to achieve efficient and accurate simulations of complex multi-physics problems, and use rocket combustion examples to motivate and evaluate our algorithms.

Projection-based reduced-order models~\cite{Lumley1997, Graham1997, Lucia2003} have proven to be effective in reducing partial differential equations (PDE)-based dynamical systems to low-dimensional manifolds and have been successfully applied in problems such as flow control~\cite{Barbagallo2012, Barbagallo2009, Barbagallo2011} and aeroelasticity~\cite{Lieu2007, Lucia2004}. When applied to complex multi-scale problems that involve transport phenomena such as convection, it is well-recognized that projection-based ROMs suffer from accuracy and stability issues. These issues may arise from the inherent lack of numerical stability of the projection method itself (e.g. Galerkin projection~\cite{Rempfer2000}), mode truncation (e.g. removal of low-energy spatial modes~\cite{Bergmann2009}), or simplifications of model equations~\cite{Noack2005}. 

Several remedies \textcolor{blue}{for these stability issues} have been proposed in the literature. For linear \textcolor{blue}{dynamical} systems, the balanced proper orthogonal decomposition technique~\cite{Rowley2005,Willcox2002} uses balancing transformations to derive numerically-stable ROMs. The use of \st{adaptive bases}\textcolor{blue}{basis adaptation}~\cite{San2015, peherstorfer2015online, PeherstorferADEIM, CarlbergAdaptiveBasis2015, EtterAdaptiveBasis2020} \st{and projection onto non-linear manifolds via deep convolutional autoencoders} has \st{also} been investigated to mitigate ROM accuracy and stability issues. Another group of studies address stability issues from the perspective of closure modeling,  \textcolor{blue}{often by} accounting for the effect of truncated \st{ROM dynamics based on the resolved ROM dynamics (analogous to the closure problem in LES)} \textcolor{blue}{basis modes~\cite{Bergmann2009, IliescuVMS2014, Parish2019} or introducing artificial dissipation terms}. Lucia et al.~\cite{Lucia2003} demonstrated the effectiveness of constructing stable ROMs by including additional artificial dissipation terms. \textcolor{blue}{Others have approached the stability problem from a controls perspective, using basis rotations~\cite{1}, eigenvalue reassignment~\cite{rezaian2020hybrid}} \st{used implicit sub-space correction and eigenvalue reassignment} to stabilize Galerkin ROMs of compressible flows \st{with shocks and vortex shedding phenomena}

\st{Variational multi-scale (VMS) closure models for projection-based ROMs have been demonstrated to offer stabilization for multi-scale problems. Parish et al. leveraged the Mori–Zwanzig (MZ) formalism to develop a closed representation of the unresolved scales. Extended to projection-based ROMs, the method is referred to as the Adjoint Petrov–Galerkin (APG) method. The Markovian first order approximation to the memory kernel yields a technique that is analogous to adjoint-stabilization in the finite element community.}

Researchers have also attempted to leverage the underlying numerical discretization to improve ROM stability. Rowley et al.~\cite{Rowley2004} pointed out that defining a physically-meaningful inner product to obtain low-dimensional manifolds (e.g. proper orthogonal decomposition bases) can yield  a quadratic reduced system that is more stable and much simpler to implement for model reduction of compressible flows. Barone et al.~\cite{Barone2008,Barone2009JCP} proposed to stabilize the reduced system by symmetrizing the higher-order PDE with a preconditioning matrix, and also highlighted the importance of formulating a proper inner product in preserving stability in the reduced system. For aeroelastic applications, Amsallem and Farhat~\cite{Amsallem2014} have shown the advantages of using the descriptor form over the non-descriptor form of the governing equations. While these methods can enable stable ROMs, they can compromise the conservative properties of the governing equations during the model reduction procedure. Afkham et al.~\cite{Afkham2020} highlighted the importance of preserving the conservative form of the governing equations in ROM development. 

Following developments in the finite element community (e.g. the Galerkin Least-Squares technique of stabilization~\cite{LSFEM}), Carlberg et al.~\cite{carlberg2013gnat,Carlberg2017}  demonstrated that minimizing the least-squares residual of the projected solution yields stabilized non-linear ROMs. This technique is referred to as least-squares Petrov-Galerkin (LSPG) projection. The GNAT method~\cite{carlberg2013gnat} extends hyper-reduction to LSPG projection.  Strategies have also been developed to explicitly enforce desirable properties such as discrete conservation~\cite{CarlbergConsvLSPG}. Grimberg et al.~\cite{GrimbergPROM2020} demonstrated improved stability, accuracy and efficiency of hyper-reduced LSPG ROMs (HPROMs) in the context of convection-dominated turbulent flows.  In practice, least-squares-based techniques have been restricted to implicit time integration schemes, as applying residual minimization to an explicit time integrator results in a test basis that is  identical to the trial basis. 

The above investigations have been demonstrated to be effective in the applications pursued in the respective publications. Many multi-scale, multi-physics contexts, such as reacting flows, further exacerbate accuracy and robustness issues  with high numerical stiffness arising from the chemical kinetics. This stiffness can lead to  Jacobian matrices with high condition numbers $O(10^{12})$, and may produce many issues even in full-order models~\cite{StoneKinetics}. For instance, a recent investigation~\cite{HuangAIAAJ2019} has identified the appearance of localized spurious oscillations near sharp, dispersed flame fronts as a major contributor to the stability issues in reacting flow ROMs. These oscillations are a consequence of under-resolution, or the inability of the ROM to resolve resolve sharp flame fronts, and can often lead to features such as negative temperatures (i.e. T $\leq$ 0 K) that terminate the calculations. A temperature limiter was required to improve ROM robustness even in relatively simple reacting flow configurations. Similar ideas of enforcing physical realizability were also employed by Blonigan et al.~\cite{BloniganHypersonics} for hypersonic flow applications in which strong temperature gradients are present.

In the present work, we develop a comprehensive framework for projection-based reduced-order model development for complex multi-scale applications to achieve improved robustness and computational efficiency. Particularly, we introduce a structure-preserving variable transformation and leverage least-squares minimization~\cite{Carlberg2017} to achieve global stabilization. To promote local stability, we enforce physical realizability on both temperature and species mass fraction fields. This method achieves discrete consistency and symmetrization at the sub-iteration level, {\color{blue} results in well-conditioned ROMs}, and allows for the use of implicit and explicit time integrators. We refer to our new formulation as the structure-preserving least-squares with variable transformation (SP-LSVT) technique. Detailed evaluations of the SP-LSVT technique and comparisons with Galerkin and LSPG projection are presented in challenging reacting flow applications.
 
The remainder of the paper is organized as follows. Section~\ref{fom} presents  the full-order model (FOM) and time discretization. Section~\ref{StandardROM} reviews the procedure for standard model reduction via Galerkin and LSPG projection. Identifying a gap in the literature, Section~\ref{proof} presents a proof of linear stability of least-squares-based ROMs. Section~\ref{SPLSPG} introduces the selection of transformed solution variables, and the procedure for SP-LSVT projection to achieve symmetrization and discrete consistency. Section~\ref{limiters} discusses a limiter-based strategy to improve local robustness. Section~\ref{results} presents numerical results  and analysis for ROMs of benchmark reacting flow problems and assesses their accuracy, robustness, and efficiency. In Section~\ref{sec:conclusion}, we provide concluding remarks and perspectives.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
